The Dark Side of Augmented Reality: Exploring Manipulative Designs in AR

Augmented Reality (AR) applications are becoming more mainstream, with successful examples in the mobile environment like Pokemon GO. Current malicious techniques can exploit these environments' immersive and mixed nature (physical-virtual) to trick users into providing more personal information, i.e., dark patterns. Dark patterns are deceiving techniques (e.g., interface tricks) designed to influence individuals' behavioural decisions. However, there are few studies regarding dark patterns' potential issues in AR environments. In this work, using scenario construction to build our prototypes, we investigate the potential future approaches that dark patterns can have. We use VR mockups in our user study to analyze the effects of dark patterns in AR. Our study indicates that dark patterns are effective in immersive scenarios, and the use of novel techniques such as `haptic grabbing' to drag participants' attention can influence their movements. Finally, we discuss the impact of such malicious techniques and what techniques can mitigate them.

==> IJHCI.DP.XR (1)/sections/conclusions.tex <==
% Conclusion
% In this paper, we presented and constructed %the construction of 
% several AR scenarios to explore how dark patterns could be implemented in the AR environment. We also included a user evaluation to examine the user perception of %their perceptions of 
% the constructed scenes of dark patterns in AR applications. We construct our scenarios using two taxonomies that include the interface and normative perspective of dark patterns. 
In this paper, we present the first comprehensive overview of possible dark pattern designs for AR ecosystems and explore the potential of such technologies in AR environments. We presented and constructed several AR scenarios to explore how dark patterns could be implemented in the AR environment. Remarkably, we construct our scenarios using two taxonomies: the interface and normative perspective of dark patterns. Additionally, we conducted a two-step user evaluation. The purpose of the user study was to determine how users perceive the constructed dark patterns scenarios in the AR application. To do so, we crafted three scenarios based on possible situations in our proposed scene construction method. The results indicate that dark patterns influence user behavior, with strong lights and objects obscuring the interface compelling users to move and prolonging gameplay. The interference of vibrations can make users miss notifications. %Accordingly, we also had a two-stage user evaluation to examine the user perception of the constructed scenes of dark patterns in AR applications. 
Our findings shed light on the users' threats from dark patterns in emerging immersive worlds, known as the Metaverse. 

==> IJHCI.DP.XR (1)/sections/dark_patterns.tex <==
% DArk Patterns
In this section, we describe in more detail the different categories of nudging according to the two taxonomies: the five dark pattern strategies by Gray~\textit{et al.}~\citep{gray2018dark}, and the normative perspectives of dark patterns by Mathur~\textit{et al.}~\citep{mathur2021makes}.


We follow the same taxonomy from Gray\textit{et al.}~\citep{gray2018dark} to categorize the different types of dark patterns (we also include examples of each category):

\begin{itemize}
    \item \textbf{Nagging}, interrupts users' desire for explanation and control. This behavior can be found in applications that interrupt users' flow, including notification messages that pop up while using the application. 
    % In the case of AR scenarios we can think more sophisticated approaches than pop-up notifications (as many AR applications already use). For example, the AR application can request the user to move to a particular spot in the room in order to prompt a specific menu item, which will allow the application to collect more information about the users' environment or diminish the users' motivation to access that menu item due to the movement involved.
    
    \item \textbf{Obstruction},  makes users spend the effort to find and understand an explanation while interacting with explanation or control facilities. We can have examples in the literature of mechanisms such as roach motel (not possible to delete an account), price comparison preview (unable to select the product brand), and intermediate currency (multiple currencies).
    % In the AR environment, the application can request the users to go to a particular physical location in the city to be able to cancel a service or account. 
    
    \item \textbf{Sneaking}, gains from the user's interaction with explanation/control facilities through hidden functions. This technique can force users to agree to accept some data collection practices to unsubscribe from a service. We can enumerate the following examples from literature: sneak into a basket, bait and switch (click a feature that requires a premium account), hidden information, and preselection.  
    % In the case of AR applications, we can see similar approaches forcing users entering a particular retail store in order to unsubscribe a service, increasing the chances of buying something in that retail store. Another example can include the use of augmented objects in the physical world to hide the real cost of items in a store.
    \item \textbf{Interface interferences} encourage explainability or control settings that the system provider prefers. This is one of the most common techniques manifested in interfaces to deceive users when (for example) they agree to the cookie consent notice (with a highlighted accept button). Under this lens, we can observe examples in the real world such as aesthetic manipulation, toying with emotion (countdown offer), false hierarchy, disguised ad (ad appears as normal content in the online newspaper or blog), and trick questions (double negative in the text).
    % In the case of AR scenarios, designers and developers are not limited by interface designs, and can further include physical objects in the surroundings to blend their dark patterns. For example, they can place important (for users) options in a menu (e.g., stop collecting personal information about them) under or behind a physical object so users can not see properly or place these options at the bottom (e.g., on the floor) so they seem less important than the rest. 
    \item \textbf{Forced action} forces users to perform an action before providing them with useful explanations or control options. For example, privacy Zuckering (send usage data preselected) and social pyramid (inviting friends to get access to a special app item).
    % In this strategy we can highlight the use of gamification as it is a common use-case of AR applications, where users are force to do repetitive tasks in order to gain points to pass to the next level of a game. However, in the AR environment, users might require to realize physical movements in order to achieve this points, with the corresponding burden.
\end{itemize}

% The analysis of dark patterns in mobile applications in~\citep{di2020ui} shows that the most common techniques in number of percentage of applications containing each technique are the following: obstruction, sneaking, and interface inferecence.
% Moreover, the nature of AR applications and its usage in the physical world can led users to not only be subjects of undesired data collection practices, but threats about their personal safety (e.g., hide real objects with virtual ones so users will bump into them).

We also follow the taxonomy suggested by Mathur et al.~\citep{mathur2021makes} that the addition of normative perspectives (from other disciplines outside HCI) on dark patterns. The aforementioned taxonomy by~\citep{mathur2021makes} shows guidelines and recommendations to analyze dark patterns outside user interface designs and apply methods grounded in normative perspectives (e.g., psychology, economics, ethics). 
% As we can observe with XR and more particularly AR scenarios such taxonomy will include new aspects that affects individuals' safety under the scope of their individual welfare



\begin{itemize}
    \item \textbf{Individual welfare.} Under this lens, a dark pattern is any interface that modifies the choice architecture to benefit the designer at the expense of the user's welfare.
        \begin{itemize}
            \item \textbf{Financial loss.} Scenarios where dark patterns cause an individual's financial loss, such as in shopping and travel websites. 
            
            % In AR applications designers can use heavy contrast parts of the real world (e.g., highlights or dark spaces) to display the extra charges when purchasing an item or displaying some discounts on physical retails, see example~\ref{}.
            \item \textbf{Invasion of privacy.} Examples of such techniques include difficult to access privacy-respecting choices (e.g., hidden options under cumbersome menus for cookie consent notices). 
            % The continuous sensing of AR applications open new possibilities to collect even more invasive information about users. These applications can force the user to move around their space (e.g., living room) in order to reply to some interface (e.g., signaling them to rotate their phone in order to visualize the notice) while the application is collecting information about the environment (e.g., point cloud, images, objects such as furniture in the room). 
            \item \textbf{Cognitive burden.} We can have examples of such behavior with interfaces that repeatedly prompt the users to accept certain choices or require users to follow cumbersome paths to unsubscribe from a particular service (e.g., via phone). 
            % In the case of AR, applications can include this cognitive burden with difficult to read interfaces (e.g., partially hidden from the users' field of view), therefore users have to move in order to be able to read the whole prompt. 
            % \item safety. This welfare consequence to users is when, in the case of AR scenarios, the dark pattern causes them to harm themselves by hidden real objects (e.g., table) under virtual scenarios, or covering their field of view and forcing them to walk without a fully perspective of the physical world around them.
        \end{itemize}
        
        % In all above scenarios we did not include other techniques that are commonly used in AR applications such as haptics and audio feedbacks. For example, the AR application design can render haptic feedback to users when the interface is prompted, annoying the users and forcing them to accept the default (or predefined) options (cognitive burden). The possibilities with AR applications are broader than other environments such as mobile applications and websites where the 2D interfaces limit the interactions and techniques that dark patterns can use.
        
        
    \item \textbf{Collective welfare.} Normative perspectives such as competition, price transparency, and trust in the market. These dark patterns can tie emotions with products in order to influence users in their purchase decision. 
    % In the case of AR scenarios, designers can display virtual objects such as violent or scary scenes in front of physical retail to influence individuals to not order or buy from that store. As we mentioned above the use of feedback such as audio or haptic when users is nearby a particular place (e.g., retail store) can trigger them emotions (fear) towards it. Therefore, users can have trust issues in similar scenarios that displays virtual objects to attract users' attention honestly. 
    
    % \item Regulatory Objectives
    \item \textbf{Individual autonomy.} Under this lens, a dark pattern is a user interface that undermines individual decision-making. The majority of dark patterns in the literature attempt to undermine individuals' autonomy. 
    % In the case of AR applications, dark patterns can enable even have a broader impact on the autonomy of individuals as such applications are related with real-world behaviours (e.g., freedom of movement). For example, a dark pattern can influence users (`trick') to follow a particular path in the physical world towards a desire destination or virtual object in the augmented space.
\end{itemize}

We omit the normative lens of the regulatory objectives as the regulatory objectives of the AR ecosystem are still under consideration and have limited legal regime scope. For example, the general data protection regulation (GDPR) regulates certain data collection and processing practices. However, despite this regulatory attempt, dark patterns are still a common technique in online services (e.g., websites). This highlights the difficulties regulators have to protect individuals' privacy, whose challenges are even direr in AR scenarios.

==> IJHCI.DP.XR (1)/sections/introduction.tex <==
% Introduction
%Extended Reality (XR) 
Augmented Reality (AR) applications seamlessly merge the virtual world into the physical world. We can also see the popularity of AR applications in smartphone applications such as Pokemon Go and Snapchat, as well as other major players in the consumer market such as AR (ARKit), Google (AR Core), and Microsoft (HoloLens)~\citep{patil2019accelerating,ar_market}. 
% For context, the AR market is predicted to reach a value market of 100 billion USD by 2024~\citep{ar_market}. 
Moreover, the ubiquity and immersion of these applications open a new space for interaction techniques and the use of these AR applications. For example, the users are not attached to a computer and can freely move in the physical world while interacting with the virtual world or augmented view~\citep{nijholt2021experiencing}. These environments raise new challenges regarding the privacy and security of users~\citep{roesner2014security,hu2021lenscap,guzman2021unravelling}.

AR technologies have the ability to integrate virtual objects with the physical world in order to change the users' perceptions of reality~\citep{chatzopoulos2017mobile}. While these applications are becoming more widespread in the commercial market, there are still limited design guidelines for the AR space. AR application design faces several changes: (i) the rapidly evolving best practices; (ii) challenges with scoping guidelines; (iii) learning by doing~\citep{drascic1996perceptual,azuma1997survey,milgram1994taxonomy,speicher2018xd}. The still newly developed AR technologies (e.g., mid-air interaction, tracking capabilities) can hinder the creation of universal design guidelines. According to Michael Nebeling~\citep{michigan_ux_xr}, we can highlight four different sources that attempt to come up with such design guidelines: (i) vendors, platform-driven; (ii) designers, user-oriented; (iii) practitioners, experience-based; (iv) researchers, empirically derived. The HCI community has been studying the effects of UX in society~\citep{ardito2014investigating,mannonen2014uncovering,rajeshkumar2013taxonomies} and from the perspective of designers and practitioners~\citep{tromp2011design,larusdottir2012big} in order to provide more responsible guidelines and mechanisms for designing UX. Moreover, the current HCI studies~\citep{machuletz2020multiple,mhaidli2021identifying,di2020ui,mathur2019dark,utz2019informed} focus on the influence of such design interfaces on user experiences (UX) and how particular design `tricks' (dark patterns~\citep{darkPatternsBrignull}) can influence the users' decisions towards behaviors desired by the designers. Following the work~\citep{gray2018dark}, we define dark patterns as `\textit{user interface designs that benefit the system instead of the user}'. 

%While there has been prior work that evaluates the AR security and privacy~\citep{hu2021lenscap,mcpherson2015no,roesner2014security}, %these works do not evaluate 
%the impact of user interfaces on the users' behaviour is rarely investigated. 
While previous research has evaluated AR security and privacy~\citep{hu2021lenscap,mcpherson2015no,roesner2014security}, the impact of user interfaces on user behavior has received little attention. 
This work aims to propose a first overview of the possible dark pattern designs that the AR ecosystem can have. It is vital %important 
to address the risks that users might face in AR applications before AR becomes established in mainstream technologies.

In the case of AR scenarios, the possibilities for dark pattern designs are even broader. They %and 
can put the users at physical risk due to the nature of displaying virtual objects in the physical world~\citep{jung2018ensuring,azuma1997survey}. Many of the current AR applications are still using mobile OS and smartphones as interaction devices~\citep{chatzopoulos2017mobile}, which can also enable traditional dark pattern designs used in other non-AR mobile applications, such as cumbersome menus to disable default settings or misleading information in the 2D menu interfaces~\citep{gray2020kind,gray2018dark,di2020ui,bosch2016tales}. 

\textit{Use case:} ``We can observe dark patterns when the application hides important content, such as menu preferences, behind the user or other physical objects, in order to keep the default values.'' In this work, we %will 
focus on interface designs that require visualization. However, more importantly, dark patterns in AR applications could be open to other interaction approaches such as haptic feedback that is rendered to nudge %avoid 
users to select an option and audio feedback that interrupts or distracts the user during their decision process.


\bparagraph{Contributions.} In this paper, we continue the research on dark patterns by exploring the possibilities of such techniques in AR environments. First, we use the scenario construction~\citep{mhaidli2021identifying} method to illustrate the possible techniques, usages, and risks that dark patterns can enable in the AR ecosystem. 
% We construct these scenarios following the taxonomy from a normative perspective~\citep{mathur2021makes}. 
This allows us to design and develop our dark pattern prototypes in new technologies, such as AR, which can be seen in other works~\citep{mathur2021makes,betten2018constructing} to predict the impact of future technologies. We analyze and describe several novel approaches to applying dark patterns in AR scenarios using the above method. 
Second, following the scenario constructions and building on top of prior works~\citep{mhaidli2021identifying,greenberg2014dark,tseng2022dark}. We use VR as a mock-up environment~\citep{prange2021priview}, where we designed an application that emulates an AR scenario in a public environment (e.g., streets). 
We use the VR mock-up for the following reasons:
\label{sec:reasons}
\begin{enumerate}
\item \textbf{AR technology limitations.} Currently, AR technology is still at its nascent stage. As such, achieving the effect of our prototype requires a significant financial investment and considerable time~\citep{rymarczyk2020technologies}. In contrast, the proposed VR environment allows us to overcome technical issues, for instance, the anchors' tracking and positioning accuracy issue -- virtual objects do not keep the same position)~\citep{yigitbas2021using}. 
\item \textbf{Examples of previous studies.} Moreover, a prior work~\citep{prange2021priview} also leverages a VR mock-up approach to evaluate their AR scenarios. %, where the authors use VR mock-ups for their proposed AR application. 
\item \textbf{Security and policy.} In our setup, we designed a street view virtual environment that simulates real streets where participants testing in the real world may encounter safety issues (e.g., crossing streets without awareness due to the AR application being tested) not only to the subject but also the bystanders, i.e., we cannot disturb the bystanders causing hassle to the urban environments. It is also important to note that putting a manipulative design in AR would violate university IRB regulations and put participants at risk.
\item \textbf{Control environment variables.} The VR mock-up scenarios allow us to have a consistent setup (e.g., lighting conditions) across all participants. This mock-up can potentially serve as digital twins~\citep{barricelli2022digital} of the reality, that is, a safe and immersive environment for evaluating the proposed manipulative designs.
\end{enumerate}
%The VR mock-up allows us to overcome %overcomes 
%limitations of current AR UX evaluation, such as ineffective input, limited field-of-view, tracking, and registration accuracy, to name but a few, % input-interactions, tracking techniques, and 
%Furthermore, VR provides a more immersive experience using smart glasses~\citep{chatzopoulos2017mobile}, and %. Moreover, it 
%provides persistent AR-like scenarios for our study. 
% Second, we design an online survey to evaluate the impact and perceptions of 75 participants on dark patterns in AR scenarios. 
% We found that the participants struggle to detect dark patterns in AR scenarios, following similar findings on more traditional UI interactions~\citep{di2020ui,utz2019informed,bongard2021definitely}.
These findings highlight the importance of guidelines and better mechanisms in AR environments where dark patterns can significantly impact users' behavior. 
% applications can monitor and collect users' surroundings, raising users' privacy threats.







==> IJHCI.DP.XR (1)/sections/related_work.tex <==
% Related work
We organize the related work into two parts according to: AR UX design, where we describe guidelines, frameworks, and techniques in the AR ecosystem; and dark patterns, where we analyze the different taxonomies and how these techniques are used in the digital world.


\subsection{AR UX design ethics}
\label{sec:devices}
AR encompasses the technologies that attempt to augment a physical environment using virtual graphics (e.g., objects, interfaces). The most common approach to displaying this augmented view is using smartphones and smart glasses or headsets~\citep{roesner2014security}. AR applications should be context-aware and adapt to the environment in which they are being used~\citep{ganapathy2013design}. For example, mobile AR applications should have the right form factor for mobile environments~\citep{ganapathy2013design}. In this work, we focus on head-mounted AR devices such as AR glasses and headsets, there are currently two forms of mainstream devices, 1) the images, generated by the device, overlap with the real world through optical see-through displays (e.g. Microsoft Hololens 2\footnote{\url{https://www.microsoft.com/en-us/hololens}}, Magic Leap\footnote{\url{https://www.magicleap.com/en-us/}}); 2) the surroundings are captured through the front camera of the VR device and then the composite image is displayed in the screen  to display the augmented view seamlessly, i.e., video see-through display (e.g. Meta Quest 2\footnote{\url{https://www.meta.com/quest/products/quest-2/}}, Pico 4\footnote{\url{https://www.picoxr.com/global/products/pico4}}). %smartphone environment, where the virtual/digital elements are rendered on the smartphone's screen using the physical perspective recorded via the smartphone's camera to display the augmented view seamlessly. 

AR technologies pose an important risk to users regarding their privacy. The continuous monitoring of the camera sensor can capture information about the users' surroundings, such as their room~\citep{roesner2014security}. Therefore, it is crucial to think about the ethical aspects of UX designs. Dark patterns and design techniques that manipulate users can pose potential risks to their privacy~\citep{gray2018dark,roesner2014security}. The ethical designs of new UI paradigms, such as AR interfaces, are of important focus in the Human-Computer Interaction (HCI) community~\citep{grimpe2014towards}. Mhaidli et al.~\citep{mhaidli2021identifying} analyze the possibilities of manipulative advertisement in XR (eXtended Reality: AR, VR, MR)~\citep{stanney2021extended}. They showcase several scenarios where advertisements target users with a misleading experience, hence influencing their decisions (e.g., by creating artificial emotions in consumers). %influencing them in their decisions (e.g., artificial emotions in consumers). 
Our work highlights the current problems that such AR-based interfaces can have and evaluate the impact of dark patterns in these immersive scenarios.

Moreover, several scholars have highlighted the risks that AR technologies can have on consumers, such as nausea, motion sickness, and safety~\citep{roesner2014security,jung2018ensuring,pierdicca2020augmented}. For example, AR applications can make users fall down when walking towards a virtual object, as they are not focusing on their surroundings~\citep{jung2018ensuring}. As we can observe in several platforms, such as Google ARCore\footnote{\url{https://developers.google.com/ar/design}} and Apple ARKit\footnote{\url{https://developer.apple.com/design/human-interface-guidelines/ios/system-capabilities/augmented-reality/}}, they consider such risks in their design guidelines and other ethical considerations. For example, virtual objects should have an appropriate size that does not force the users to walk backward to see them in their totality, see Figure~\ref{fig:related_work:googleAR_safety}.

\begin{figure}[t]
  \centering
      \includegraphics[width=0.5\columnwidth]{figures/related_work/googleAR_guidelines_safety.pdf}
      \caption{A screenshot captured from the Google ARCore design guidelines. We can see a person tripping over a physical (real) object while walking backward and using an AR application. }
      \label{fig:related_work:googleAR_safety} 
\end{figure}

Several works emphasize the importance of UX design in order to provide ethical applications~\citep{gray2018dark,ethical_design,ethical_design_karr}. Although any design can have the effect of influencing the user~\citep{oinas2009persuasive,rajeshkumar2013taxonomies}, the abusive use of `malicious' techniques, such as dark patterns, should be restricted~\citep{gray2018dark}. Dark patterns are an example of abusive interface designs that influence the users' welfare and their behavior (e.g., artificially creating a sense of scarcity of flight tickets on online websites).

\bparagraph{Haptics for XR.} Haptic stimuli has been a common approach in mobile devices (smartphones, wearables) to provide a notification channel for mobile applications~\citep{schaub2015design,mehta2016privacy,luk2006role}. We can see haptic feedback broadly used in games, where the controllers provide haptic sensations when the virtual player crashes with another virtual object (e.g., car crash in the game)~\citep{tamborini2006role}. Haptics is also a common technique in other XR scenarios, such as VR games~\citep{bermejo2021exploring}. Haptic devices will play an important role in AR experiences, where the haptic stimuli can enhance the realism and immersion of AR~\citep{bermejo2021survey}. Moreover, haptic stimuli can evoke different emotions according to the feedback displayed (e.g., frequency and intensity of the haptic feedback)~\citep{rovers2004him,obrist2015emotions,vekemans2021motus,eid2015affective}. Users can associate particular valence and arousal according to the received haptic stimuli~\citep{yoo2015emotional,vekemans2021motus}. In~\citep{yoo2015emotional}, the authors showed that the frequency of tactile icons affects people's perception of emotions. Therefore, haptic feedback and the emotions it evokes can be used in the design of dark patterns for XR applications. We focus on certain dark pattern designs in AR with haptic feedback, as it is a commonly used channel to interact with users and can be implemented in current wearables. 

Similarly, the audio sensory channels can be used to enhance the realism and immersion of AR experiences~\citep{chatzopoulos2017mobile}. Although these audio techniques can be considered in the design of dark patterns, we believe that audio should be tested in a physical environment (e.g., streets) and not VR mockups, so noises from the outside world can reduce the performance of audio interaction in AR. In this work, we focus on haptic and visual approaches and consider audio cues as part of future work.




\subsection{Dark patterns}
Dark patterns can be found in highly diversified 
%very different 
environments, such as online media, games, and social networks~\citep{gunawan2021comparative,fitton2019creating,utz2019informed,mathur2019dark,machuletz2020multiple}. The ubiquitous %ubiquity 
presence of dark patterns becomes even direr when we think about AR environments. As we will see in this paper, the mixed relation between physical (real) and virtual objects in AR applications enables new approaches to `tricking' users. Thus, addressing such threats becomes relevant. 

Brignull~\citep{darkPatternsBrignull} gathers on his website a collection of real-world examples of dark patterns commonly used in websites and mobile applications. The website aims to raise users' awareness of dark pattern practices and constructs a reported dataset of widely used dark patterns. Brignull proposes an initial taxonomy of 12 elements according to the user interface `trick', such as \textit{privacy Zuckering} that tricks users into sharing more personal information. 

Several works propose taxonomies to categorize various %the different 
dark pattern techniques~\citep{conti2010malicious,gray2018dark,mathur2021makes} in a broader sense. Conti~\textit{et al.}~\citep{conti2010malicious} categorize the dark pattern techniques as malicious interface design approaches. They categorize 11 interface designs that can be problematic for users. For example, obfuscation hides interface elements from users. Gray~\textit{et al.}~\citep{gray2018dark} propose a taxonomy using a similar data collection for their corpus as Brignull (tweets from users). They introduced new dark patterns on top of the categories of Brignull, such as nagging and forced action. The latter requires users to perform a specific action repeatedly in order to continue. The authors increase the number of categories in a later version~\citep{gray2020kind} by collecting users' posts about dark patterns on Reddit. Outside the interface design techniques, we can mention the work by~\citep{mathur2021makes} that proposes the addition of normative perspectives in the analysis and categorization of dark patterns. These normative perspectives focus their taxonomy on disciplines outside the HCI community, such as psychology, economics, and ethics. 

% The prior works on dark patterns main focus on UI for more traditional systems (e.g., websites, mobile apps) can be restricted by the aforementioned taxonomies. 
The prior works on dark patterns mainly focus on the UIs of traditional systems (e.g., websites, mobile apps), which can be restricted by the aforementioned taxonomies. Studies, e.g., \citep{mathur2021makes,greenberg2014dark} show %Works, such as~\citep{mathur2021makes,greenberg2014dark} shows 
new perspectives that are not limited to %of 
user interfaces and can be extended to %used for 
new environments, such as AR. For example, the use of haptics, as a dark pattern technique, is not usually included in prior taxonomies. Additionally, %and 
only some works~\citep{mhaidli2021identifying,greenberg2014dark} illustrate more techniques to manipulate users' decisions.

Our work serves as the groundwork for the design of dark patterns in the emerging AR scenarios, especially in the following two taxonomies from these works: Gray~\textit{et al.}~\citep{gray2018dark}, Mathur~\textit{et al.}~\citep{mathur2021makes}, and Greenberg~\textit{et al.}~\citep{greenberg2014dark}. We leverage %use 
these taxonomies as they are the most recent. They further highlight % and includes 
UI perspectives~\citep{gray2018dark} and illustrate how dark patterns can affect the users' privacy~\citep{mathur2021makes}. Remarkably, %Although 
we extend these taxonomies, due to the mobility characteristics of AR as well as %and 
other essential user-oriented factors, such as safety and privacy. %with a new categories such as safety. 






==> IJHCI.DP.XR (1)/sections/research_challenges.tex <==
% Discussion
The results of our scenario construction and user study show the impact of dark patterns in AR scenarios. Visual-based manipulations (lighting and object interference) affect the participants' responses. Moreover, there is an impact on the participants' time to solve the maze when using these dark pattern designs, as the participants that did not agree with sharing their personal information (try to read the whole message) spent more time solving the maze. In the case of haptic grabbing, we saw an impact of the haptic stimuli on participants' movements. The haptic feedback nudges the participants toward the direction of the controller rendering the stimuli.




% Our outcomes reveal the importance and the challenges that users, designers, and regulators can face when dark pattern techniques are implemented in AR ecosystems. 

% \subsection{Implications}

% The constructed scenarios illustrate the impact that dark patterns can have in future AR applications. We build our proposed AR scenarios on top of the most up-to-date dark pattern taxonomies from an interface and normative perspective. These proposed scenarios can help designers and regulators overview the possibilities of such `malicious' techniques in AR applications. The community can use these scenarios to evaluate further the effects of dark patterns in AR applications, such as raising their awareness and informing them about the risks of dark patterns. 

% % Our findings show that users are unaware of malicious designs in AR scenarios, which reinforces the importance of better-informed designs and more strict regulations when designing interfaces. This paper can be used as the groundwork taxonomy of dark patterns for immersive scenarios such as AR, where researchers and practitioners can refine and extend with more cases (e.g., dark pattern techniques implemented in haptic feedback).

% The proposed dark patterns are plausible scenarios that can be implemented with the current AR technology. However, more sophisticated technologies that include more photorealistic experiences can increase the effect of dark patterns on users' behaviour. For example, sneaking techniques can take advantage of the sophistication of AR technologies when a `fake/alternative' image or text is displayed on top of real objects to show a different price or brand. The trends in the AR ecosystems are going forward more realistic experiences (including haptic feedback). Therefore, dark patterns will likely utilise such capabilities to expand the techniques to influence users. For example, dark pattern techniques can use realistic haptic feedback to influence users using approaches not yet implemented with current technologies (i.e., beyond interface designs).

% However, AR applications are still not widespread, and the interaction capabilities with such environments are still far from perfect. Furthermore, there are still several constraints regarding devices to visualise virtual objects (e.g., smart glasses) and even more limitations when users interact with the environment (e.g., hand-gesture recognition, gaze-based interaction). Therefore, dark patterns for AR are still in their early stage. Our proposed scenarios and online study showcase hypothetical yet practical approaches that might or might not change when AR becomes more mainstream.

% With this work, we aim to bridge the gap between current technologies for AR and the possibilities of dark patterns in AR described in the constructed scenarios. We describe the future challenges and approaches that such manipulative scenarios can pose in the development of AR applications. In the following paragraphs, %sections, 
% we highlight the main research challenges and intervention mechanisms that could be implemented to counterbalance the use of dark patterns.


\subsection{Dark Patterns in immersive experiences}

Novel %New 
and more effective dark patterns can be implemented in AR due to the immersive and realism of the environments. These improved user experiences can enable more sophisticated approaches to alter users' behaviors. In comparison with other traditional user interfaces (e.g., desktops, phones), dark patterns in AR can have a greater impact on the users' decision process~\citep{mhaidli2021identifying}. Most of these traditional approaches meticulously design user interfaces to `trick' and influence users without their awareness~\citep{gray2018dark}. In the case of AR applications and hyper-realistic virtual objects, the users will not be able to distinguish them from physical ones~\citep{ruth2019secure}. \textit{How %then 
can we tell users that a hyper-realistic virtual object is not genuine without hindering the user experience and immersion?}

Besides the realism of virtual objects, the immersiveness and interactivity of these environments can also impact the effectiveness of dark patterns. 
% For example, in AR applications, dark patterns can use multi-modal techniques (e.g., visual, audio, haptic) to increase the effect of dark pattern designs on users' behaviors. 
Similar to the effects of audio on the shoppers' buying intentions in retail stores~\citep{milliman1982using}, AR applications can create immersive dark patterns using visual, audio, and haptic feedback. The AR ecosystem can augment the effect of dark patterns into influencing users' behaviors. It is necessary to %There is also the need to 
analyze the main factors influencing users when dark patterns (using visual, audio, and haptic) are applied in AR environments, and how can we protect users in these immersive experiences.

Finally, AR applications allow users to interact with their interfaces using more natural approaches (natural interactions)~\citep{shatilov2019emerging}. These natural interactions can also be the subject of dark pattern techniques. 
For example, when a user clicks a UI button via gaze or using the index fingertip as a controller. In this case, a dark pattern can hide (hijack) the authentic cursor behind a virtual object and use a fake cursor to click another UI interface (e.g., an ad banner)~\citep{lee2021adcube}. These virtual elements, being inserted during the input interactions of users, require framework-driven regulations %to be controlled by frameworks 
within the AR ecosystem. Following the work in~\citep{lee2021adcube}, future AR platforms should consider the defense against dark pattern attacks, whose techniques are implemented during the interaction process (e.g., cursor movement). 

Moreover, we can see dark patterns in AR as interface-dependent, where the different screens/field of view options can have different implications for the implementation of dark patterns. This, together with the multi-modal nature of AR applications (visual, auditory, and haptic), can open new approaches for the design of dark patterns beyond traditional systems such as smartphones and computers.  


% However, AR applications are still not widespread, and the interaction capabilities with such environments are still far from perfect. Furthermore, there are still several constraints regarding devices to visualise virtual objects (e.g., smart glasses) and even more limitations when users interact with the environment (e.g., hand-gesture recognition, gaze-based interaction). Therefore, dark patterns for AR are still in their early stage. Our proposed scenarios and online study showcase hypothetical yet practical approaches that might or might not change when AR becomes more mainstream.

With this work, we aim to bridge the gap between current technologies for AR and the possibilities of dark patterns in AR described in the constructed scenarios. We describe the future challenges and approaches that such manipulative scenarios can pose in the development of AR applications. In the following paragraphs, we highlight the main research challenges and intervention mechanisms that could be implemented to counterbalance the use of dark patterns.


\subsection{Privacy of AR}

The sensing requirements of AR applications, such as capturing camera frames, open privacy risks that differ significantly from traditional interfaces (i.e., desktops, phones). As mentioned in previous works~\citep{guzman2021unravelling,de2019security,roesner2014security}, the scanning capabilities of devices used in AR ecosystems raise several privacy concerns and challenges to protecting users' privacy. For example, the spatial information captured from these devices (point clouds) can leak information about the personal space of a user (e.g., bedroom size) and objects (e.g., furniture) belonging to a particular user~\citep{guzman2021unravelling}. Designers can develop dark pattern techniques that force users into capturing more information about their surroundings without their awareness. Obviously, some of these designs are only intended to drive/change specific user behaviors and are not malicious or intended to manipulate users. However, they can still raise privacy concerns among users.

% In AR scenarios, users will have even more challenges to fully understand the data being collected (sensed data), as well as the purpose and impact of the data collection. The captured data from multiple sensors can become %play 
% an even bigger threat than ever before, especially when the collected information is aggregated. Third parties (e.g., manufacturer of devices, application developers, or cloud services) can infer even more detailed information about the user profiles, for instance, furniture retailers capture users' physical behaviour (e.g., gaze attention) when shopping in real grocery stores)~\citep{guzman2021unravelling}.

% Most of the current AR applications installed in our smartphones lack protection techniques to minimize or obfuscate the identity of bystanders (individuals that might be captured by the smartphone's camera while using an AR application). In~\citep{hu2021lenscap} the authors propose a system that requires a policy manager to allow AR applications to share captured data from sensors (e.g., spatial information) to external servers such as third party clouds. The framework will manage how each application share the collected data, with privacy-by-default and privacy-by-design policies~\citep{langheinrich2001privacy}. AR technologies are also characterized by their collaborative features, where multiple users can create, visualize, interact, and play with virtual objects~\citep{ruth2019secure}. In these contexts, the potential privacy risks come from the user's device side and other users in the AR scenario (multiplayer). We can have a future of AR applications where dark patterns are not only created by app designers but by other users of the application. For example, virtual objects in specific physical locations can affect users behaviour, such as the obfuscation of a real store. In~\citep{ruth2019secure}, the authors propose a secure control framework to manage the content sharing capabilities in multi-user environments of AR applications. This framework can also enable the control of dark pattern techniques in AR environments when are implemented by other users with malicious intentions. 


% The solutions mentioned above can prevent privacy leakages, which are independent of the dark pattern techniques used for such purposes. %while independent of the dark pattern techniques used for such purposes. 
% As we have seen in previous works~\citep{matte2020cookie}, despite the regulations (e.g., the GDPR) serve to protect users' personal information, the use of malicious techniques are still widespread counteracting the effectivness of such regulations~\citep{bermejo2021website,utz2019informed}. 


% The experience we have with privacy regulations such as data protection and cookie consent notices ~\citep{bermejo2021website, matte2020cookie} show us that dark pattern techniques



\subsection{Safety of AR}

Malicious designs can cause critical risks to the safety of users in AR environments~\citep{lebeck2017securing, roesner2014security}. 
For instance, AR cues become the obfuscation visually to a particular street in the physical world. When a user is crossing a road, the obfuscation can put the users in danger due to reduced awareness of incoming vehicles. %For example, the obfuscation of a particular physical street, when users are walking to force them to walk another route, can put them in danger (e.g., incoming vehicles from the hidden street). 
In comparison with other traditional interfaces, dark patterns can become a more prominent threat for users of AR applications. 

The management of content and visual output of virtual objects in AR applications can guarantee %ensure 
a safer environment for users~\citep{ruth2019secure, lebeck2017securing}. 
These security and safety risks should be mitigated with platforms and regulations that control how the visual output is displayed to users \citep{james-lam} in a harm-free manner. 
%and controlling there is no harm to users. 
% Authors in~\citep{lebeck2017securing} propose an AR platform to control the visual output of AR applications according to specific policies leveraging context awareness of the users. These context-aware policies limit the virtual content, in which %that 
% users can view %visualize 
% in their AR applications. Moreover, the visual output of virtual objects can also come from other users of the platforms (collaborative environments). Therefore, the control of virtual outputs should also consider %these 
% multi-user environments, considering that %with the challenges of multi-creation environments raise. 
% multi-user creation in collaborative environments are emerging. Finally, non-visual feedback cues, %output 
% such as audio and haptic, should be included %considered 
% in the scope of context-aware policies.



\subsection{Intervention mechanisms}

In this section, we discuss the results in the scope of the problems that dark pattern arises from previous works in more traditional environments (desktop, smartphone)~\citep{bongard2021definitely,di2020ui,bermejo2021website,utz2019informed,mathur2019dark}. %, 
We connect the previous works regarding the issues with AR~\citep{roesner2014security,lebeck2017securing,ruth2019secure,de2019security,langheinrich2001privacy}, to %and 
our findings in the realm of dark patterns and AR.  
Intervention mechanisms aim to provide individuals with the tools and protection techniques they need to protect their personal information from malicious designs such as dark patterns. These intervention techniques can be developed for either the user or the environment. For example, regulators will enforce and intervene in scenarios where dark patterns can put users with AR applications at risk. %the safety of users when using AR applications (e.g., more control on AR map apps).



\bparagraph{Increasing awareness.} Our results show that users are not fully aware of the manipulation techniques used in dark pattern designs in AR, following previous work relevant to traditional interfaces~\citep{di2020ui,utz2019informed,bongard2021definitely}. 
% that users are not fully aware of the manipulation techniques used in dark pattern designs. 
Moreover, even when users are aware of design `tricks', they do not fully understand the manipulation or its purpose (e.g., what type of information is being collected). 
In the case of AR applications, individuals' awareness and concerns regarding dark patterns are even lower due to the lack of experience with AR applications and the novelty of this environment (as we discussed in this paper), i.e., the users' technology literacy to the evolving malicious techniques. 
The addition of feedback cues, such as audio and haptic, to raise users' concerns (e.g., warnings~\citep{gray2018dark}) when a particular suspicious design is being used, can increase user awareness and their understanding of dark patterns. 
However, warning techniques can reduce their effectiveness with time (users get habituated to them)~\citep{akhawe2013alice}. Mechanisms that increase users' awareness of dark patterns should change with time (e.g., different feedback modes, not always active) so as to keep their effectiveness. 



\bparagraph{Education and training.} Our results show that participants with some experience with AR applications had higher chances to detect dark patterns in our study. Moreover, following the above statement about user awareness and concerns regarding dark patterns, we believe that sustainable mechanisms to further educate users about the threats of dark patterns and how these can be detected can increase the individuals' self-protection abilities. For example, the combination of the above warning techniques, together with better education and training about the threats of dark patterns (e.g., privacy and attention-grabbing mechanisms), can allow users of AR applications to become more aware of these malicious designs.

\bparagraph{Counteracting dark patterns in the digital space.} As the results of our study show, dark pattern techniques can have a significant impact on users' behaviors. For example, attention-grabbing techniques using haptic feedback change the participants' movements in the maze, and interference approaches using lighting conditions and objects affect their responses. Moreover, these manipulative designs will overcome the countermeasures of several frameworks that protect users from malicious AR output (e.g., notifications that cover users' field-of-view)~\citep{lebeck2017securing,roesner2014security}. These frameworks should also include more control over the interface design and output of virtual elements and allow users to report and customize the AR output to limit manipulative designs such as the ones studied in this paper. Also, these countermeasures should consider the interface used to interact with AR, as we can see an interface-dark pattern correlation in the design of manipulative techniques.

% Dark patterns are usually present in our online daily lives~\citep{mathur2019dark, utz2019informed, gray2018dark}. We can see them when buying in online stores~\citep{mathur2019dark} and when a cookie consent notice obtains %request 
% our consent~\citep{utz2019informed}. Several works study the implementation of mechanisms, such as nudging to counterbalance the effects of dark patterns~\citep{bermejo2021website,acquisti2017nudges,nouwens2020dark}. 
% Other solutions aim to eliminate the dark patterns (e.g., cookie consent notices~\citep{nouwens2020dark}). 
% Ethical design approaches, such as privacy-by-design~\citep{gray2019ethical}, should also consider %include 
% the interface designs, bringing %so there is more 
% higher transparency during the development of services.

% However, the ubiquity of dark patterns on online services can hinder the implementation of intervention techniques that modify the current behaviour of dark patterns without monetary incentives (to business) or regulations. In the case of AR applications, these applications' ubiquity and mobile nature increase the challenges to developing tools to eliminate dark patterns. 

As we described in our scenario construction section, the possibilities for designing AR interfaces are humongous compared to more traditional interfaces (desktops, smartphones). Even when the dark patterns are somewhat analogous to well-recognised designs from these traditional interfaces, individuals are not fully aware of them. Moreover, AR applications not only pose privacy threats to users~\citep{de2019security} but also endanger their safety~\citep{roesner2014security} when malicious techniques are applied with such a purpose (e.g., hiding real objects from users' view~\citep{leao2011altered}). Therefore, regulations, economic incentives, and ethical designs should play a mutually important role in counteracting and controlling the dark patterns in AR applications. 



\subsection{Limitations of our study}

In terms of limitations, using the same physical environment can result in carry-over effects, which can impact the effects of dark patterns. 
Nevertheless, our study offers a realistic environment to study the effects of dark patterns in AR. One outcome we could not assess with the current study is the long-term effect of such dark patterns on users' everyday behavior. Our participants were from our university campus and they have some experience with AR or XR applications. Meanwhile, because our participant group was comprised of students, they would be especially concerned about the questions posed in our scenario, and all participants demonstrated a high regard for privacy issues. Thus, the participants were hesitant to reveal them; however, different groups may have varying levels of concern/non-concern/awareness/prudence regarding perceived privacy violations. Therefore, our results should be considered in the context of the participants we recruited.

We use the haptic vibroactuator device embedded in the Oculus controller for our experiment. One of the reasons we chose this option was to account for the fact that many of the most common AR headsets currently in the industry use hand controllers with vibration feedback for interactions (refer to Section~\ref{sec:devices}). We acknowledge that further studies in the haptic feedback direction should consider other stimuli areas and different haptic devices, for example, haptic gloves~\citep{nam2008smart,koyanagi2005development}, weight simulation~\citep{wang2022vibroweight} and thermal feedback~\citep{maeda2019thermodule}.

Due to the considerations mentioned in Section~\ref{sec:reasons}, we use VR mock-up to simulate AR. The emulated environment will inevitably differ slightly from the actual AR situation; for instance, the fidelity of the real environment will be higher than the street of the VR simulation, and the real world with digital overlays will provide more immersive environments to the user. If conditions permit, future researchers can construct a photo studio, e.g., a dark pattern sandbox, to conduct AR experiments for the sake of investigating user behavior in the context of dark patterns and AR, ensuring user safety and controlling environmental variables.

The current user study presents a limited type of dark pattern that can potentially appear in AR environments when they are widely adopted. The future version of this work will include more experiments and AR scenarios to provide more in-depth technical details in this direction. 

% In this paper, we aim to provide the first taxonomy of dark patterns in AR scenarios. Although we construct our scenarios using previous taxonomies~\citep{mathur2021makes,gray2018dark}, we need to reinterpret some of the definitions, use cases, and extend them for immersive experiences. We also restrict the prototypes to reduce the redundancy of dark pattern examples and focus on simple scenarios, so the participants in the online study can easily (if any) detect and identify these `malicious' approaches. We acknowledge that the design space of the constructed dark pattern scenarios can be broader. In this work, we aim to construct these scenarios following current dark pattern trends so the participants can identify these mechanisms.


% % Future extensions of this work will include more AR-based dark pattern techniques, such as haptic and audio feedback.

% Another limitation of our categorization is the lack of an in-depth study of current dark pattern practices in AR applications. We do not include such classification of instances of dark patterns due to the still premature ecosystem of AR applications and the still limited capabilities (e.g., the smartphone is mainly used as the primary device in AR). Future extensions of this work will aim to categorize the current dark pattern used in AR applications accordingly. 

% As for the online study, we analyzed the effects of dark patterns by watching a prerecorded video. The above can limit the ecological validity of the results in more realistic scenarios such as using the application in the real world. This might be a reason that the participants have difficulties finding the dark patterns. Our study aims to provide a first overview of the effects of dark patterns in AR applications on a broader number of participants. Future works will include a more in-depth study conducted in an in-lab user study to compare our results. We use a 15-seconds length for the recorded videos as the scenarios are simple use-cases that include only the necessary interfaces to showcase the dark patterns. In real-world scenarios, and following results from other works~\citep{di2020ui,utz2019informed,bosch2016tales} the complexity of interfaces will difficult even more the identification of dark patterns by users.


% As we mentioned above, the current dark patterns we address in our taxonomy do not include techniques implemented using haptic or audio feedback. Although, these feedback approaches are becoming more important in the AR ecosystem as they increase the realism of the user experience~\citep{bermejo2017survey}.







\subsection{Future work}


In this work, we present novel dark pattern designs for AR according to current technologies. As revealed by %we have observed in 
our results, the use of alternative modalities, such as haptic feedback, can open new possibilities for dark pattern designs beyond traditional UIs~\citep{greenberg2014dark}. Similarly, audio feedback and more sophisticated haptic approaches could be used in future designs of dark patterns for AR. 
% In all the prototypes, we did not include other techniques in AR applications, such as haptics and audio feedback. For example, the AR application design can render haptic feedback when the interface is prompted, annoying the users and forcing them to accept the default (or predefined) options (cognitive burden). 
We do not include more sophisticated approaches in this work as the current technologies for haptic rendition are still in their infancy. Meanwhile, commercial approaches can be mainly found as %in 
vibroactuators devices, known as %in 
gamepads, smartphones, and smartwatches~\citep{bermejo2021survey}. The possibilities with AR applications are broader than the traditional counterparts, %in other environments 
such as mobile applications and websites, where non-AR interfaces limit the interactions and techniques that dark patterns can use.

Future extensions of this work will include studying diversified devices (e.g., Microsoft HoloLens, Google Glass) available in the wide spectrum of the AR ecosystem (i.e.,, low-end to high-end devices). Moreover, we will %should 
extend our current work with the study of multi-modalities for dark patterns, such as haptic, audio, and visual, which can provide new perspectives on the design of dark patterns for AR, following futuristic scenarios such as the ones enumerated in~\citep{mhaidli2021identifying,greenberg2014dark,tseng2022dark}.

% Future extensions of this work will include classifying current AR applications (e.g., smartphones, HoloLens) using the taxonomy in this paper. The classification of the dark pattern used in the current AR application can also provide new perspectives and categories that were not included in our taxonomy. We will include in future versions of this work the scenario construction and implementation of haptic and audio feedback use-cases as they are the distinctive feature of AR compared to other environments such as websites. We have already included some examples in this work. However, we will conduct a more extensive evaluation of the possible techniques and devices available in AR applications (e.g., smart glasses, haptic devices), their feasibility, and their effect on users' behaviour. We will require the use of an in-lab user study -- to be able to render, for example, haptic feedback.

Finally, VR technologies and technologies in the extended reality (XR) have been getting traction recently with the announcement of the Facebook introduction of `meta'\footnote{\url{https://about.fb.com/news/2021/10/facebook-company-is-now-meta/}}. The metaverse will open new challenges to preserve users' privacy~\citep{lee2021internet}. In addition to that, ChatGPT\footnote{\url{https://openai.com/blog/chatgpt}}, an artificial intelligence chatbot built on top of the GPT-3 language model and introduced by OpenAI in November 2022, may lower the barrier to creating malicious manipulation in the future. In future applications, such chatbots are likely to be integrated with XR creation, and through such chatbots, everyone will be capable of creating AR instances more easily and conveniently in the future. These are the emerging research topics that future researchers should investigate. Future work will also include an extensive analysis of dark patterns in these virtual environments to avoid threats such as abusive ad service providers~\citep{lee2021adcube}.



==> IJHCI.DP.XR (1)/sections/scenario_construction.tex <==
% Scenario construction
In this section, we utilize \textit{scenario construction} -- motivated by previous works~\citep{mhaidli2021identifying,speicher2018xd,di2020ui} to evaluate the dark pattern techniques that can be applied in AR applications. 
This approach can help us understand the possible impact of dark patterns and explore potential problems with such techniques in AR. 


Scenario construction is an effective tool to analyze the impact (in our case) of dark patterns in AR technologies. Previous works have used this method to describe and evaluate the impact of future technologies~\citep{mhaidli2021identifying,betten2018constructing,reijers2018methods} and their ethical impacts on society~\citep{mhaidli2021identifying}. In our case, we construct each scenario by assigning one of the existing categories in the aforementioned dark pattern taxonomies and illustrating the manipulative mechanisms.


In our case, the proposed scenarios are used to highlight the potential privacy threats that dark patterns can arise on users in AR environments. 
% Following the aforementioned taxonomies, we describe several different scenarios where dark patterns can have a potential impact on individuals' behaviour~\citep{weinmann2016digital,acquisti2005privacy}. 
We aim to construct scenarios that are easy to understand, and %that are easier to understand and 
reflect techniques that are similar to the ones currently used in other environments (e.g., websites, mobile applications), so we can have more accurate examples~\citep{wright2014ethical}. Although the commonly used approaches in non-AR-based interfaces, such as highlight buttons, can also be used in many instances of the AR ecosystem, we propose more innovative techniques that combine AR applications' mixed (physical-virtual) nature. We also constructed the scenarios according to popular applications, such as games and furniture applications, to achieve a more realistic analysis of the effects of dark patterns in AR environments. We use the following prompts to develop our initial set of scenarios, where dark patterns can influence the users' decisions in AR environments:

\begin{itemize}
    \item Can we use existing dark patterns techniques in AR?
    \item How can we take advantage of AR's immersion, ubiquity, and mobility to increase the effects of dark patterns?
    \item How the dark pattern technique can influence users' decisions?
\end{itemize}


%These prompts to revise and iterate over the initial set of scenarios (following the aforementioned taxonomies and features of AR). 
These prompts were revised and iterated over the initial set of scenarios (following the aforementioned taxonomies and features of AR). 
We condense some of the following scenarios into real prototypes to analyze the users' perceptions of dark patterns or manipulative designs in
AR interfaces. %the AR interface.


\subsection{AR features}
Following previous works~\citep{mhaidli2021identifying,barnes2016understanding,roesner2014security,betten2018constructing,bosch2016tales,greenberg2014dark,speicher2018xd}, we identify these defining characteristics of AR that differ from other modalities (e.g., websites): immersiveness, pervasiveness, and realism. We enumerate the above characteristics according to the current technologies, and we acknowledge that this may vary in the future. 
These traits, which come with AR environments by nature, can pose novel risks~\citep{roesner2014security} to users compared to the dark pattern taxonomies that are currently used for UIs in mobile apps~\citep{di2020ui,bosch2016tales} and websites~\citep{utz2019informed,mathur2019dark,machuletz2020multiple}. 
%These characteristics, inherited naturally in AR environments, can pose novel risks ~\citep{roesner2014security} to users in comparison with the current dark pattern taxonomies that are relevant to UIs in mobile applications~\citep{di2020ui,bosch2016tales} and websites~\citep{utz2019informed,mathur2019dark,machuletz2020multiple}.  
%These features natural in AR environments can pose novel risks~\citep{roesner2014security} for users in comparison with the current dark pattern taxonomies related to UI in mobile applications~\citep{di2020ui,bosch2016tales} and websites~\citep{utz2019informed,mathur2019dark,machuletz2020multiple}.  

\bparagraph{Immersive.} In the context of AR, immersive can be seen as a seamless %seamlessly 
blend of the virtual world with the physical surroundings. The digital enhancements or virtual objects are smoothly rendered over the physical or real world without users' awareness. The users will believe that %both 
digital and virtual are part of the physical (real) scene. The level of immersion will depend on the technologies used to render the digital world and how the users interact with it. For example, most of the current mobile AR applications are displayed on the screen of a smartphone which reduces the immersive as users have a screen-through device, and the interactions are simple touches on display. Despite the current technological limitations, AR is still more immersive than non-AR mediums~\citep{lombard2001interactive}. Therefore, it is important in the context of dark patterns to include constructed scenarios and examples that use immersive AR applications.


\bparagraph{Pervasively.} The ubiquity nature of AR applications can be an important feature that is always around the users. We can showcase an example with Google Glass or similar AR smart glasses and the privacy issues that appear around them due to the continuous sensing of the user's environment~\citep{roesner2014security}. By being worn or used anywhere and anytime, AR applications open new privacy threats to users, such as collecting their surroundings (e.g., friends, and personal spaces). Although other modalities pose a privacy threat when dark pattern techniques are implemented, in the case of AR, the risks and possible harms are direr due to the ubiquity nature of AR.


\bparagraph{Realism.} We can relate realism to immersiveness as both combined can significantly improve the overall user experience in AR environments. A realistic and immersive AR application can pose a risk to %in 
the safety of users, as they will have issues discerning %to discern 
digital from real~\citep{jung2018ensuring}. Dark pattern techniques can involve scenarios where the users are completely unaware of their surroundings, leading them into unsafe situations (e.g., crossing the road without checking the traffic light). 
% Moreover, realistic AR application in combination with malicious designs can be used for product placement (e.g., overlay another brand product on top of the real one) without users noticing. Another example is an AR-based approach to insert other content (e.g., product) between real ones in a similar way some ads pass as actual news in online newspapers. 
The danger that dark patterns leverage AR technologies to distort the users' reality and influence their behavior is very relevant. %The danger that AR technologies when using dark patterns to distort the users' reality and influence their behaviour is very relevant.
%As a way of synthesizing 
To synthesize the AR scenarios, we use the above distinctive features of AR environments 
% in the dark pattern taxonomies described in more detail 
in the following sections.



% \begin{figure}[t]
%   \centering
%     % \begin{subfigure}[b]{0.49\columnwidth}
%         \includegraphics[width=0.5\columnwidth]{figures/scenario_construction/scenario_financial_loss.png}
%         \caption{Sneaking/Financial loss example.}
%         \label{fig:scenario_construction:financial_loss} 
%     % \end{subfigure}
%     \caption{Example of dark pattern in an AR scenario. The figure illustrates an example of sneaking or financial loss, where the interface hides the extra charges by displaying them in a very bright area of the field-of-view, where users cannot properly see it without extra movement.}
%     \label{fig:scenario_construction}
% \end{figure}



% \subsection{Interface perspective}
\subsection{Scenarios}

% There are several works that focus the study of dark patterns from an interface perspective~\citep{darkPatternsBrignull,gray2018dark,di2020ui,mathur2019dark}, where dark pattern designs are implemented in UIs, and more general perspectives of dark patterns~\citep{mathur2021makes}, which includes the addition of normative perspective into the spectrum of dark patterns. 
As we have described above, AR applications go beyond more traditional interfaces, and the taxonomies from an interface perspective can limit the possibilities of dark patterns in AR. We can still sample a few scenarios according to some categories of this taxonomy. Still, %but 
following other works, such as~\citep{greenberg2014dark,mhaidli2021identifying}, we can observe that AR `dark' designs can go beyond traditional interfaces. Figure~\ref{fig:scenario_construction_new} shows some examples of our scenario construction.




% has been studied in several worls~\citep{,}
% We first define several scenarios according to the taxonomy by Gray~\textit{et al.}~\citep{gray2018dark} that focuses on interface design techniques:


% \begin{itemize}

    % \item \textbf{Nagging,} interrupts users' desire for explanation and control. This behaviour can be found in applications that interrupt users' flow, including notification messages that pop up while using the application.  
    % \begin{quotation}
    % % \hspace{-0.95cm}
    % \textit{ An online travel agency uses an AR application to provide users with a more immersive experience while booking hotels. However, the application uses audio feedback (e.g., seaside pleasant sounds) to affect users decisions when booking a particular room with seaside views. The other non-seaside view rooms do not include any sound or music.} 
    % \end{quotation}

    % \cparagraph{Construction Process.} Background music and other types of audio feedback can greatly influence users while shopping~\citep{milliman1982using}. As we can experience in retail clothing stores, background music can affect our shopping behaviour~\citep{milliman1982using}. The immerse nature of AR applications can allow us to provide users with visual feedback and audio and haptic. In this case, we construct an AR application that uses sound and music to influence users during their booking process. The background sounds of the sea together with background music provide users with a more natural and pleasant experience when investigating a particular hotel room.

    \bparagraph{Obstruction-forced action,} these techniques make use of blocking or forcing particular actions on users (e.g., window pop-ups, mandatory registration to read a news website), drive or guide users to do some behavior. 
    
    
    \begin{quotation}
    % \hspace{-0.95cm}
    \textit{A retail store has an AR application that requests users to move to a particular physical location (e.g., a store) to unsubscribe from %for 
    their newsletter. The retail store uses this unsubscribing method to force users to go to their physical store, raising the possibility that the users might buy something once inside the store.} 
    \end{quotation}
    
    \cparagraph{Construction Process.} 
    Under this lens, we can observe the potential burden on users due to walking to a particular location or the change in their path due to virtual obstacles. Moreover, this technique can be combined with other mechanisms, such as sneaking or obstruction, to force users to move to a particular physical location. In contrast, the different mechanisms can enable more sophisticated dark patterns~\citep{roesner2014security}.
    %Under this lens, we can observe besides the potential burden of users due to walk to a particular location or the changing on their path due to virtual obstacles. Moreover, this technique can work in combination with other mechanisms such as sneaking or obstruction to force the user to move to a particular physical location, where the other mechanisms can enable more sophisticated dark patterns~\citep{roesner2014security}.

    
    
    
    % The AR application can request the users to go to a particular physical location in the city to be able to cancel a service or account. In this scenario, the application can force the users to go to a particular physical location or do a particular (difficult) movement to cancel the service. The obstruction in AR applications can imply some physical or cognitive burden in their approaches. They might require users to either move physically to a location or force them to do some repetitive task similar to the forced action technique but with the goal of canceling a service.
    
        
    % \item \textbf{Sneaking,} gains from the user's interaction with explanation/control facilities through hidden functions. This technique can force users to agree to accept some data collection practices to unsubscribe from a service. We can enumerate the following examples from literature: sneak into a basket, bait and switch (click a feature that requires a premium account), hidden information, and preselection.  
    
    % \begin{quotation}
    % \textit{A brand creates a hyperrealistic AR application that can overlay realistic virtual objects in the physical world. Users cannot discern the real objects from the virtual generated ones. The application can use this realistic experience to overlay %their 
    % virtual objects on top of other rival brands. The users will %make then 
    % purchase the items without noticing the brand is different. }
    % \end{quotation}
    
    % \cparagraph{Construction Process.} We can have examples of such sneaking behaviour in online services, such as online newspapers, where media content is introduced in the news feed~\citep{sheehan2013controversies}. This media content is then seen as a news publication without the readers' awareness that it is a sponsored content ad. In the AR ecosystems, applications can include augmented objects in the physical world to hide the real cost of items in a store. 
    % The ubiquity of AR scenarios can lead to a situation where our AR perspective is completely different from the real world -- for example, in a smart city, all the AR banners hide the real brands and names of stores in our field of view. This can open new markets where the best bid gets the digital AR banner. 
    
    
    \bparagraph{Interface interference,} 
    % encourages explainability or control settings that the system provider prefers. 
    this is one of the most common techniques manifested in interfaces to deceive users when (for example) they agree to the cookie consent notice (a highlighted accept button)~\citep{bermejo2021website}. 
    % Under this lens, we can observe examples in the real world such as aesthetic manipulation, toying with emotion (countdown offer), false hierarchy, disguised ad (ad appears as normal content in the online newspaper or blog), and trick questions (double negative in the text).
    
    \begin{quotation}
    \textit{An online retail store develops an AR application to allow customers to buy items by focusing on them in the physical world using the AR field of view. When the consumers want to select the delivery method, the interface uses the physical world objects to obfuscate the delivery method without extra charges. Without being noticed properly, the consumers will choose the delivery method (with extra charges) within the ones they can see.} %The consumers, without noticing, will select the delivery method (with extra charges) within the ones they can see.}
    \end{quotation}
    
    \cparagraph{Construction Process.} To construct this scenario, we first consider the applications that use highlighted buttons or hidden menu options (using links instead of buttons) to force users to select the desired (by third parties) options~\citep{bermejo2021website}. 
    In the case of AR scenarios, interaction designs are no longer limited to 2D interfaces. More importantly, designers and developers can further implant dark patterns in physical objects to blend the user's surroundings. 
    %In the case of AR scenarios, designers and developers are not limited by interface designs and can further include physical objects in the surroundings to blend their dark patterns. 
    % For example, they can place important (for users) options in a menu (e.g., stop collecting personal information about them) under or behind a physical object. Therefore users can not see properly or place these options at the bottom (e.g., on the floor), and these options seem less important than the rest. 
    
    
%     \item \textbf{Forced action,} forces users to perform an action before providing them with useful explanations or control options. For example, privacy Zuckering (send usage data preselected) and social pyramid (invite friends to get access to a special app item). 
    
%   \begin{quotation}
%     \textit{And advertisement company uses the AR interface to display ads at the entrance of the user's work. When the user passes near the augmented ad, it shows a full video of the advertised product.}
%     \end{quotation}
    
%     \cparagraph{Construction Process.} 
%     In this strategy, we can highlight the use of gamification as it is a common use-case of AR applications, where users are forced to do repetitive tasks to gain points to pass to the next level of a game~\citep{gray2018dark}. However, in the AR environment, an advertisement company can force users to see or realize action that requires either users' movement or are displayed in their surroundings, forcing them to watch the ad. These approaches will incur users to realize physical movements to achieve these points, with the corresponding burden.

     \bparagraph{Safety.} The pervasive, mobile, and realistic natures of immersive scenarios in AR applications open new threats to the safety of users. 
            
        \begin{quotation}
        \textit{An AR game uses realistic virtual interfaces and objects to provide an immersive experience. This application looks %is so 
        real and natural to users. As a result, the users %that they 
        cannot distinguish the physical objects from the virtual ones. The application can then uses these virtual objects to create virtual obstacle near the physical ones. Once the user tries to avoid the virtual obstacle will trip over %with 
        the physical one in the vicinity.}
        \end{quotation}
        
        \cparagraph{Construction Process.} To construct this scenario, we follow previous works~\citep{roesner2014security,lee2021adcube}, where authors discuss the risks to user safety %the safety risks 
        that immersive technologies such as AR can have on users. Contrary to more traditional environments such as websites, in the case of AR scenarios, the dark pattern causes them to harm themselves by hiding real objects (e.g., a table) under virtual scenarios, or covering their field of view, and consequently forcing them to walk with an incomplete perspective of the physical world around them. 
        
    \bparagraph{Associative dark patterns.} These dark patterns can tie emotions to products in order to influence users' purchase decisions.  
    
        \begin{quotation}
        \textit{A perfume brand uses the augmented view of an AR application to display the perfume, being purchased by other people like close friends and influencers, through the lens of AR. %display the perfume of other people's perfume in the camera frame. 
        That is, the %The 
        application associates the person with perfume. A user might be unsure about what perfume to buy, but the application will display the above perfume-person association %perfume-person 
        in the buyer's surroundings. This social association, as augmented information, will influence the buyer to buy a specific perfume related to someone in the buyers' social circle or someone (bystander) that he/she likes.} 
        %(e.g., clothes, appearance). }
        \end{quotation}
        
        \cparagraph{Construction Process.} To construct this scenario, we follow the associations that brands utilize to sell their products, such as campaigns that use models and particular features that trigger some emotions in buyers~\citep{kidane2016factors}. 
        % . Clothing, perfumes, and accessories are usually advertised through campaigns that use models and particular features that trigger some emotions in buyers~\citep{kidane2016factors}. 
        For example, watches usually are associated with luxury and beauty. 
        % Moreover, designers of AR can display virtual objects such as violent or scary scenes in front of physical retail to influence individuals not to order or buy from that store. 
        The use of feedback, such as audio or haptic, whenever users are nearby a particular place (e.g., a retail store) can trigger emotions (e.g., fear) towards it. 
        % Therefore, users can have trust issues in similar scenarios that display virtual objects to attract users' attention honestly. 
    
% \end{itemize}

Moreover, the nature of AR applications and their usage in the physical world can lead users to become not only subjects of undesired data collection practices, but also threats to %about 
their personal safety~\citep{jung2018ensuring}. For example,  (e.g., hiding %hide 
real objects with virtual ones so users will bump into them - so-called diminished reality~\citep{herling2012pixmix,leao2011altered}). %Similarly 
Similar to their findings (though in VR) in the work~\citep{dao2021bad}, users are unaware of their surroundings or the virtual objects (original, fake copy, interactions with virtual objects)~\citep{lee2021adcube}.


\begin{figure}[t]
  \centering
        \includegraphics[width=1\columnwidth]{figures/scenario_construction/scenario_construction_new.png}
        \caption{Examples of dark patterns in AR scenarios. a)\ding{172} The virtual interface on the ground obstructs the user's way forward; a)\ding{173} A virtual interface that appears in an inappropriate location, forcing the user to walk to a special location to unsubscribe; b)\ding{172} A virtual pricing icon blocks out the physical price tag; b)\ding{173} A blinding halo of light obscures the information on the interface; c)\ding{172} The virtual item (house) is unnecessarily bulky in the users’ view. As such, it enforces the user to step backward in order to visualize the whole item. As a result, the user may be at risk of hitting objects in the blind spot of the field of view; c)\ding{173} User crashes into a tangible table to avoid the virtual lamp; d)\ding{172} Users see virtual celebrities using luxury goods while in a luxury store; d)\ding{173} Some mood-altering (e.g., horror) sounds and vibrations (head-mounted AR controllers or some wearable devices) can influence the user choices.}
        \label{fig:scenario_construction_new}
\end{figure}


% \begin{figure}[t]
%   \centering
%     \begin{subfigure}[b]{0.49\columnwidth}
%         \includegraphics[width=0.9\columnwidth]{figures/scenario_construction/scenario_financial_loss.png}
%         \caption{Financial loss example.}
%         \label{fig:scenario_construction:financial_loss} 
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\columnwidth}
%         \includegraphics[width=0.8\columnwidth]{figures/scenario_construction/dp_object.png}
%         \caption{Privacy loss example.}
%         \label{fig:scenario_construction:obstruction}
%     \end{subfigure}
%     \caption{Examples of dark patterns in AR scenarios. Figure~\ref{fig:scenario_construction:financial_loss} illustrates an example of financial loss. The interface %, where the interface 
%     hides the extra charges by displaying them in a very bright area of the user's field of view (FOV), where users cannot properly see them %it 
%     without adjusted FOV by extra movements. %with extra movement. 
%     Figure~\ref{fig:scenario_construction:obstruction} depicts a %an 
%     privacy loss where a physical object obfuscates several options of the notice.}
%     \label{fig:scenario_construction}
% \end{figure}


% \subsection{Normative perspective} We also follow the taxonomy in~\citep{mathur2021makes} that suggests the addition of normative perspectives (from other disciplines outside HCI) on dark patterns. The aforementioned taxonomy by~\citep{mathur2021makes} shows guidelines and recommendations to analyze dark patterns outside user interface designs and apply methods grounded in normative perspectives (e.g., psychology, economics, ethics). Following this taxonomy, as we can observe with XR and, more particularly, AR scenarios, such taxonomy will include new aspects that affect individuals' safety under the scope of their welfare that propose the following scenarios:



%     \begin{itemize}
%         \item \textbf{Individual welfare.} We can group techniques under this lens that threaten the users financially (e.g., money or privacy loss). We also extend the current category with an additional perspective that refers to the safety of users in AR environments, see Figure~\ref{fig:scenario_construction:financial_loss}.
        
%         \begin{itemize}
        
%             \item \textbf{Financial loss.} Scenarios where dark patterns cause an individual's financial loss, such as in shopping and travel websites. 
            
%             \begin{quotation}
%             \textit{An online retail store has developed an AR application where customers can buy items. The application uses state-of-the-art techniques to analyze the frame and place different virtual lighting effects on top of the prices of physical objects. Therefore, the users cannot fully see the product's actual price when purchasing them. }
%             \end{quotation}
            
%             \cparagraph{Construction Process.} To construct this scenario, we use a similar approach to~\citep{lee2021adcube}, where designers use tricks to hide users' interactions in VR (e.g., fake cursor). Motivated by this work, we believe that designers of AR applications can use future technologies to realistically add virtual lighting effects (darker, brighter) to make difficult visibility of %to difficult the visibility of 
%             specific areas in the user's FOV. %of the field of view. 
%             In another example, designers of AR applications can use heavy contrast parts of the real world (e.g., highlights or dark spaces) to display the extra charges when purchasing an item or to display some discounts on physical retails, see Figure~\ref{fig:scenario_construction:financial_loss}.
            
%             \item \textbf{Privacy loss.} Examples of such techniques include difficult-to-access privacy-respecting choices (e.g., hidden options under cumbersome menus for cookie consent notices). 
            
%               \begin{quotation}
%                 \textit{A retail store that sells furniture has developed an AR application to display its %their 
%                 products in the buyers' rooms. However, the application forces users to scan their whole room before visualizing the virtual furniture.}
%                 \end{quotation}
                
%                 \cparagraph{Construction Process.} The continuous sensing of AR applications opens new possibilities to collect even more invasive information about users~\citep{hu2021lenscap,guzman2021unravelling}. These applications can force users to move around their space (e.g., living room). %These applications can force the user to move around their space (e.g., living room). 
%                 For example, to reply to some interface, the user has to rotate their phone to visualize the complete notice~\citep{lam2019m2a}. Meanwhile, the application is collecting information about the environment (e.g., point clouds, images, physical objects such as its rival's furniture)~\citep{guzman2021unravelling}. 
            
%             \item \textbf{Cognitive burden.} We can have examples of such behaviour with interfaces that repeatedly prompt the users to accept filtered choices at default 
%             %certain choices 
%             or require users to follow cumbersome paths to unsubscribe from a particular service (e.g., via phone). 
            
%             \begin{quotation}
%             \textit{A newsfeed AR application automatically forces users to its monthly subscription by trialing the application. their monthly subscription to try the application. 
%             When users want to unsubscribe from the service, the application forces them to read the menu interface to interact in very poorly %poor 
%             lighted locations of users' surroundings. The application can detect the locations in the users' field of view where the text and buttons are harder to read, such as against the sunlight or in very dark areas of the frame. }
%             \end{quotation}
            
%             \cparagraph{Construction Process.} We construct this scenario following similar applications that include cognitive burden with difficult-to-read interfaces in websites. For example, cumbersome and long text that requires users' inputs continuously to unsubscribe from a service.
    
            
        %     \item \textbf{Safety.} The pervasive, mobile, and realistic natures of immersive scenarios in AR applications open new threats to the safety of users. 
            
        %     \begin{quotation}
        %     \textit{An AR game uses realistic virtual interfaces and objects to provide an immersive experience. This application looks %is so 
        %     real and natural to users. As a result, the users %that they 
        %     cannot distinguish the physical objects from the virtual ones. The application can then uses these virtual objects to create virtual obstacle near the physical ones. Once the user tries to avoid the virtual obstacle will trip over %with 
        %     the physical one in the vicinity.}
        %     \end{quotation}
            
        %     \cparagraph{Construction Process.} To construct this scenario, we follow previous works~\citep{roesner2014security,lee2021adcube}, where authors discuss the risks to user safety %the safety risks 
        %     that immersive technologies such as AR can have on users. Contrary to more traditional environments such as websites, in the case of AR scenarios, the dark pattern causes them to harm themselves by hiding real objects (e.g., table) under virtual scenarios, or covering their field of view and
        %     consequently forcing them to walk with an incomplete perspective of the physical world around them. 
        %     %forcing them to walk without a full perspective of the physical world around them.
            
        % \end{itemize}
        
        
% \begin{figure*}[t]
%   \centering
%     \begin{subfigure}[b]{0.39\columnwidth}
%         \includegraphics[width=\columnwidth]{figures/scenario_construction/dp_interface_frame.png}
%         \caption{Interface interference.}
%         \label{fig:scenario_construction:screenshots:interface}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.39\columnwidth}
%         \includegraphics[width=\columnwidth]{figures/scenario_construction/dp_sneaking_frame.png}
%         \caption{Sneaking.}
%         \label{fig:scenario_construction:screenshots:sneaking}
%     \end{subfigure}
%      \begin{subfigure}[b]{0.39\columnwidth}
%          \includegraphics[width=\columnwidth]{figures/scenario_construction/dp_obstruction_frame.jpg}
%         \caption{Obstruction.}
%         \label{fig:scenario_construction:screenshots:obstruction}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.39\columnwidth}
%          \includegraphics[width=\columnwidth]{figures/scenario_construction/dp_forced_action_frame.png}
%         \caption{Forced action.}
%         \label{fig:scenario_construction:screenshots:forced}
%     \end{subfigure}
%      \begin{subfigure}[b]{0.39\columnwidth}
%          \includegraphics[width=\columnwidth]{figures/scenario_construction/dp_safety_frame.png}
%         \caption{Safety.}
%         \label{fig:scenario_construction:screenshots:safety}
%     \end{subfigure}
%     \caption{Screenshots of the five scenarios with dark patterns. For example in~\ref{fig:scenario_construction:screenshots:safety} the virtual item is so big in the users' camera view that it forces the user to walk backwards in order to visualize the whole item.}
%     \label{fig:scenario_construction:screenshots}
% \end{figure*}



% \begin{figure}[t]
%   \centering
%     \begin{subfigure}[b]{0.3\columnwidth}
%         \includegraphics[width=\columnwidth]{figures/scenario_construction/no_dp_interface_frame.png}
%         \caption{Scenario A.}
%         \label{fig:scenario_construction:screenshots:no_dp:s1}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.3\columnwidth}
%         \includegraphics[width=\columnwidth]{figures/scenario_construction/no_dp_forced_action_frame.png}
%         \caption{Scenario B.}
%         \label{fig:scenario_construction:screenshots:no_dp:s2}
%     \end{subfigure}
%      \begin{subfigure}[b]{0.3\columnwidth}
%          \includegraphics[width=\columnwidth]{figures/scenario_construction/no_dp_safety_frame.png}
%         \caption{Scenario C.}
%         \label{fig:scenario_construction:screenshots:no_dp:s3}
%     \end{subfigure}
%     \caption{Screenshots of the three scenarios without any dark pattern. Figure~\ref{fig:scenario_construction:screenshots:no_dp:s1} depicts the same scenario as the obstruction but without any dark pattern. Figure~\ref{fig:scenario_construction:screenshots:no_dp:s2} illustrates the forced scenario but without any dark patterns (users are not required to move). Figure~\ref{fig:scenario_construction:screenshots:no_dp:s3} shows the safety scenario with appropriate object size.}
%     \label{fig:scenario_construction:screenshots:no_dp}
% \end{figure}
       
%     \item \textbf{Collective welfare.} Normative perspectives reflect %, such as 
%     competition, price transparency, and trust in the market. These dark patterns can tie emotions with products in order to influence users in their purchase decisions.  
    
%     \begin{quotation}
%     \textit{A perfume brand uses the augmented view of an AR application to display the perfume, being purchased by other people like close friends and influencers, through the lens of AR. %display the perfume of other people's perfume in the camera frame. 
%     That is, the %The 
%     application associates the person with perfume. A user might be unsure about what perfume to buy, but the application will display the above perfume-person association %perfume-person 
%     in the buyer's surroundings. This social association, as augmented information, will influence the buyer to buy a specific perfume related to someone in the buyers' social circle or someone (bystander) that he/she likes.} 
%     %(e.g., clothes, appearance). }
%     \end{quotation}
    
%     \cparagraph{Construction Process.} To construct this scenario, we follow the associations that brands utilize to sell their products, such as campaigns that use models and particular features that trigger some emotions in buyers~\citep{kidane2016factors}. 
%     % . Clothing, perfumes, and accessories are usually advertised through campaigns that use models and particular features that trigger some emotions in buyers~\citep{kidane2016factors}. 
%     For example, watches usually are associated with luxury and beauty. 
%     % Moreover, designers of AR can display virtual objects such as violent or scary scenes in front of physical retail to influence individuals not to order or buy from that store. 
%     The use of feedback, such as audio or haptic, whenever users are nearby a particular place (retail store) can trigger emotions (e.g., fear) towards it. 
%     % Therefore, users can have trust issues in similar scenarios that display virtual objects to attract users' attention honestly. 
    
%     % \item Regulatory Objectives
%   \item \textbf{Individual autonomy.} Under this lens, a dark pattern is a user interface that undermines individual decision-making. The majority of dark patterns in the literature attempt %attempts 
%   to undermine individuals' autonomy.  
   
%   \begin{quotation}
%     \textit{Imagine a map application that uses the AR view to guide users through the physical world. %However, the application uses object recognition and the user's location (e.g., GPS) to guide him/her through particular streets where specific retail stores.  
%     %These retail stores bid in an auction process similar to the current ads ecosystem to get the control to guide the users near their stores, increasing their visibility in the real world.
%     However, the application uses object recognition and the user's location (e.g., GPS) to guide him/her through a particular route enclosing particular retail stores. Indeed, the retail stores in such a route bid in an auction process analogue to the current ads ecosystem, to leverage AR navigation service to maximize their visibility to AR users, such as seeing their brands and potentially visiting their stores. }
%     \end{quotation}
    
%     \cparagraph{Construction Process.} We follow the current dark pattern approaches that aim to diminish the individuals' autonomy. In the AR ecosystem, dark patterns can even have a broader impact on the autonomy of individuals, i.e., the freedom of user movements / nudging the users picking narrow choices of paths. %as such users' freedom of movement. 
%     For example, a dark pattern can influence users (`trick') to follow a particular path in the real world towards the desired destination by a third party.
% \end{itemize}

% We omit the normative lens of the regulatory objectives, as the regulatory objectives of the AR ecosystem are still under consideration and have limited legal regime scope. For example, the general data protection regulation (GDPR) regulates certain data collection and processing practices. However, despite this regulatory attempt, dark patterns are still a common technique in online services (e.g., websites). 
% It is worth highlighting %This highlights 
% the difficulties regulators have to protect individuals' privacy, whose challenges are even direr in AR scenarios.





\subsection{Limitations}

Although we construct our scenarios using previous taxonomies~\citep{mathur2021makes,gray2018dark}, we need to reinterpret some of the definitions, and use cases, and extend them for immersive experiences. We also restrict the prototypes to reduce the redundancy of dark pattern examples and focus on simple scenarios, so the participants in the online study can easily (if any) detect and identify these `malicious' approaches. We acknowledge that the design space of the constructed dark pattern scenarios can be broader. In this work, we aim to construct these scenarios following current dark pattern trends so the participants can identify these mechanisms.

Another limitation of our categorization is the lack of an in-depth study of current dark pattern practices in AR applications. We do not include such classification of instances of dark patterns due to the %still 
premature ecosystem of AR applications and the %still 
%limited capabilities (e.g., the smartphone is mainly used as the primary device in AR). 
limited capabilities of headset devices, i.e., smartphones are the primary testbed of AR. 
Future extensions of this work will aim to categorize the current dark pattern used in AR applications accordingly. 

Using these scenarios, we developed an initial set of AR scenarios where dark pattern techniques are implemented. We avoid overly complicated AR examples to provide a subset of distinct scenarios that are easy to understand. The following section describes the user study, using VR environments as mockups of scenes being constructed, that analyzes the effects of dark patterns.


% \subsection{Synthesis: manipulation in AR}
% The manipulation techniques enumerated above can produce a far more profound impact on users in AR scenarios than more traditional interfaces, such as websites and mobile apps.
% %our construction.
% %The manipulation techniques enumerated above can have a more profound impact on users in AR scenarios. 
% For example, the realism and ubiquity of AR can have a more amplified effect on users' emotions than non-AR interfaces. The artificial experience created by AR can lead users to believe what they see is all real (including the digital dark patterns), generating more intense emotions~\citep{quesnel2018you}. The emotional manipulations can be leveraged even more in AR due to its pervasiveness. 
% Furthermore, dark %Dark 
% patterns can be deployed in very different contexts, such as social gatherings with friends and purchasing items in a grocery. %when surrounded by friends or when going grocery shopping. 
% In general, the combination of dark patterns and AR technologies can distort reality with the great danger that may involve. Using these scenarios, we developed an initial set of AR scenarios where dark pattern techniques are implemented. We avoid overly complicated AR examples to provide a subset of distinct scenarios that are easy to understand. The following section describes the user study, using VR environments as mockups of scenes being constructed, that analyzes the effects of dark patterns on users' behaviour.

% Using these scenarios, we developed an initial set of AR prototypes where dark pattern techniques are involved. We revised the proposed scenarios to avoid redundant and overly complicated AR scenarios in order to provide a subset of distinct scenarios that are easy to understand. In the following section, we describe the user study that analyze the effects of dark patterns in this subset of scenarios.





% \subsection{Selected dark patterns and AR scenarios}

% We selected five techniques from the aforementioned taxonomies to study whether the participants will identify the dark patterns in AR scenarios (see Figure~\ref{fig:scenario_construction:screenshots}). Each of these techniques showcases simple yet efficient dark pattern approaches that can influence users in AR environments. Motivated by previous works~\citep{di2020ui,mathur2019dark,moser2019impulse} that evaluated screenshots and videos to recognize dark pattern techniques in e-retail stores and mobile applications, we created our prototypes and video sources for our online experiment. We use the same use-case application example for each of the following scenarios. This allows us to simplify the environment and have only one degree of freedom according to each different dark pattern technique used.


% List of scenarios for dark patterns, we first categorize the proposed scenarios using the Gray~\textit{et al.}~\citep{gray2018dark} taxonomy and in brackets, the normative perspective categorization, see Figure~\ref{fig:scenario_construction:screenshots}:

% \begin{itemize}
%     \item \textit{Interface interference}. A button behind a physical object. In this scenario the interface will hide some of the buttons behind real/physical objects so the users either are required to move to see the complete interface or just interact with the available and visible buttons~\citep{gray2018dark}. Figure~\ref{fig:scenario_construction:screenshots:interface} illustrates a traditional menu interface, where one of the options is hidden behind the monitor.
%     % \item Informative text not in the field of view of the user (it requires the user to move in order to see the text)
%     \item \textit{Sneaking (financial loss)}. Overlay augmented view on top of the real text to hide the real brand of a product (similar to~\citep{billinghurst2001magicbook}). The AR prototype (\ref{fig:scenario_construction:screenshots:sneaking}) hides the real cost of an article (item from a website) using a fake price tag (augmented view).
    
%     \item \textit{Obstruction (Cognitive burden)}. Virtual text on the floor that requires the user to look down in an uncomfortable position~\citep{evangelista2021xrgonomics}. In~\ref{fig:scenario_construction:screenshots:obstruction} the prototype displays the menu interface on the floor.
    
%     \item \textit{Forced action (cognitive burden}, invasion of privacy). Continuous rotating of the user to continue the menu navigation (e.g., rotating the user in order to see deeper menu options), motivated by the work~\citep{lam2019m2a}. Figure~\ref{fig:scenario_construction:screenshots:forced} displays the menu options further from the users' position, so they have to move in order to read and press one of the available options (blue buttons on the right side of the image).
    
%     \item \textit{Safety (cognitive burden)}. Virtual object too big in the view so requires the user to walk backward~\citep{jung2018ensuring,dao2021bad}. The virtual object is rendered so big on the users' field of view (from the camera in our prototype) that it forces them to walk backwards in order to interact and fully visualize the item.
    
% \end{itemize}


% We also include three different scenarios similar to interface interference and obstruction but without any dark pattern technique involved in the design, see Figure~\ref{fig:scenario_construction:screenshots:no_dp}. These three scenarios can allow us to measure the effects of dark patterns as we will compare their responses in the absence of such techniques in the AR scenario.




% We implement the above scenarios using ARKit\footnote{\url{https://developer.apple.com/augmented-reality/}} and simple virtual objects (text, 3D basic objects such as cubes) using reality composer\footnote{\url{https://developer.apple.com/augmented-reality/tools/}} to render the different AR scenarios, following the same philosophy for rapid prototyping of AR in~\citep{leiva2020pronto}. We use an iPad Pro 2020 11 inches as the main device and record each AR scenario in the offices of our university.



% \subsubsection{Recording Methodology}
% We screen-record each of the above AR-based scenarios for 15 seconds, where we try to highlight the dark pattern techniques in each scenario by interacting with them. Some of the scenarios require the user to move around the physical environment. For example, we will move around (rotating) to navigate the menu in forced action. We choose 15 seconds as an appropriate duration to identify the possible dark patterns (if any). The scenarios include only basic interfaces and objects to facilitate the understanding and identification of users.



% Our study was guided by the visualization of traditional dark pattern approaches (where participants have seen them in other environments such as websites) in a more controlled environment. The visualization of specific aspects corresponding to dark patterns allows us to study the effects of AR visualizations on isolation. The length of the videos tries to accommodate a reasonable visualization time to detect the dark patterns (if any) without being too long for the participants. 











==> IJHCI.DP.XR (1)/sections/user_study.tex <==
% User Study
We carried out a two-stage user study to analyze in detail the effects of dark patterns in AR scenarios.

%\subsection{Ecological validity}

%The VR mockup scenarios allow us to have a consistent (e.g., lighting conditions) setup across all participants. Moreover and following prior work~\citep{prange2021priview}, where the authors use VR mockups for their proposed AR application. The VR environment also allows us to overcomes anchors' tracking issues, such as drifting (virtual objects do not keep the same position). In our setup, we designed a street view virtual environment which emulates a real street, but without the possible safety issues that participants might face in the real-world (e.g., crossing streets without awareness due to the AR app being tested).

% \textcolor{blue}{Due to social distancing requirements for COVID-19 pandemic, outdoor user testing with head-mounted AR devices is not practical. Therefore, we used Oculus Quest 2 to build three mock-up virtual reality (VR) scenarios for our user study.}


%\subsection{Ethical considerations}

%The study was carried out following the IRB regulations of our university. We carefully followed the social distancing requirements and made sure to disinfect %desinfect 
%the whole setup after each session to comply with all the COVID-19 pandemic related rules in our country. 

\subsection{Participants and apparatus}

\bparagraph{Participants.} We recruited %the 
\textcolor{black}{15 (10M/5F, $\overline{age}$ = 24.27),} participants using a consecutive sample. All the participants have a high education level or higher. Seven participants reported having some XR experience, such as VR or AR games. All participants self-reported an emphasis on privacy, with a mean value of 4.53 ($SD = 0.74$, on a 5-point Likert scale). All participants reported good vision and come from Asian cultural backgrounds. 


\bparagraph{Apparatus.} We built our mockup virtual scenarios using an Oculus Quest 2 and its controllers (1832 $\times$ 1920 pixels per eye, 120 Hz, 90 FOV). We developed the three scenarios using Unity\footnote{\url{https://unity.com/}} and the SteamVR plugin\footnote{\url{https://assetstore.unity.com/packages/tools/integration/steamvr-plugin-32647}}. The application was running on a stationary PC.

\subsection{Design and structure} 

 Before reporting the design study, we describe the different implemented AR applications according to the subset of scenarios described during the scenario construction (Section~\ref{sec:scenario_construction}). 

\begin{figure}[t]
  \centering
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\columnwidth]{figures/user_study/virtual_maze_top.png}
        \caption{Aerial view.}
        \label{fig:user_study:virtual_maze:aerial}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=0.9\columnwidth]{figures/user_study/virtual_maze_side.png}
        \caption{Side view.}
        \label{fig:user_study:virtual_maze:side}
    \end{subfigure}
    \caption{Screenshots of the virtual maze. In Figure~\ref{fig:user_study:virtual_maze:aerial}, we can see an aerial view, the notices will pop up at specific locations in the maze. 
    Figure~\ref{fig:user_study:virtual_maze:side} depicts the side view of the virtual maze.}
    \label{fig:user_study:virtual_maze}
\end{figure}


\begin{figure}[t]
  \centering
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=0.92\columnwidth]{figures/user_study/vr_maze_light.png}
        \caption{Lighting inter.}
        \label{fig:user_study:conditions:light}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=0.94\columnwidth]{figures/user_study/vr_maze_object.png}
        \caption{Object inter.}
        \label{fig:user_study:conditions:object}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\columnwidth}
        \includegraphics[width=0.9\columnwidth]{figures/user_study/vr_maze_haptics.png}
        \caption{Haptic nagging.}
        \label{fig:user_study:conditions:haptic}
    \end{subfigure}
    \caption{Screenshots of the different conditions that participants will see during the experiment. We can observe the obfuscated words in Figures~\ref{fig:user_study:conditions:light} and \ref{fig:user_study:conditions:object}. Figure~\ref{fig:user_study:conditions:haptic} illustrates the haptic condition, where the notification is placed on one side of the street.}
    \label{fig:user_study:conditions}
\end{figure}


\bparagraph{Conditions.} Three scenarios were designed to explore dark patterns in AR. These dark pattern design %dark design 
approaches are a sampling of what the future of dark patterns in AR could be. These %This 
approaches are still grounded by the current technologies in AR environments. We use VR as a tool to immerse participants in the respective scenarios, as these VR mockups can emulate the AR environment in the virtual scene (see Figure~\ref{fig:user_study:virtual_maze}).

% malicious for MAR are a sampling of what could be done in MAR environments with the current technologies and hardware. 

\begin{itemize}

    \item \textbf{Lighting interference.} In this scenario, we follow similar design approaches: %than 
    interface interference, sneaking, and obstruction, as proposed in previous works~\citep{gray2018dark,darkPatternsBrignull}, where UI elements (e.g., buttons with different colors) influence the users' decisions. In this case, the message will hide specific words in the questions using strong lighting conditions (e.g., halo), see Figure~\ref{fig:user_study:conditions:light}. The participants cannot see clearly the whole question and they are forced to move around in order to visualize the complete notice.
    
    \item \textbf{Object interference.} Similar to the previous interference, in this case, we use physical objects (street lamps in our VR mockup) to hide specific words in the messages or notifications (Figure~\ref{fig:user_study:conditions:object}). %notice. 
    We showcase two possible approaches that AR developers can use to manipulate users' decisions with a combination of virtual and physical objects.
    
    \begin{figure}[t]
     \centering
        \includegraphics[width=1\columnwidth]{figures/user_study/Haptic_Exp_Design.png}
        \caption{\textcolor{black}{Illustration setup for %Details of 
        haptic grabbing scenes. Each participant experiences triggers and notification interfaces for aligned/opposite directions in each scene.}}
        \label{fig:user_study:Haptic_Exp_Design}
    \end{figure}
    
    \item \textbf{Haptic grabbing.} This condition indicates the impacts of haptic feedback, as rendered by VR controllers, %that In this scenario we use haptic feedback (rendered in the VR controllers) 
    to grab the participant's attention to the right or left of the virtual map, producing corresponding stimuli on the left- or right-hand controller, respectively (Figure~\ref{fig:user_study:conditions:haptic}). We designed two scenarios, see Figure~\ref{fig:user_study:Haptic_Exp_Design}: \textit{scene 1}, we evaluate the effects of haptics on participants' movements; \textit{scene 2}, we study the effect of positive/negative haptic stimuli to grab participants' attention towards the notice. 
    % to evaluate the effect of haptics in participants' movements (haptic in the left or right controller) and positive/negative haptic stimuli to grab users' attention towards the notification (haptic always on the side of the notification), see Figure~\ref{fig:user_study:Haptic_Exp_Design}.
    %rendering the stimuli on the right or left controll respectively. 
    Attention grabbing can interfere not only with the decision-making process of users but -- in this case -- reduce the probability of viewing %to see 
    the notices on the virtual map. 
    Motivated by the proposed scenario in~\citep{greenberg2014dark}, we evaluate the efficacy of haptic feedback to control users' movements in our VR mockup. For example, this could allow new manipulative designs that leverage %can use 
    haptic notifications to prevent %avoid 
    users from looking at a nearby physical store. %s. 
    In our study, the participants were told that they would receive haptic feedback at particular locations in the virtual maze and with different controllers (left or right).
    
    %The virtual environment has a number of interactive cube objects, with each side showing a number of options, all of which are the same, and the user cannot detect if they have missed observing the face of the cube. Whether the haptics of the interactive virtual objects will avoid longer interactions. We designed to variants of this scenario, one with positive (pilot study) haptic feedback and other with negative haptic feedback. At each location where there is a question displayed in the virtual maze, the haptic fill either render the feedback on the right or left side according to a counterbalanced ordered.

\end{itemize}

According to prior studies~\citep{acquisti2005privacy}, privacy is an important concern of users and one of the main goals of %targets in 
dark pattern designs~\citep{mathur2021makes,bermejo2021website,di2020ui,gray2018dark}. For both lighting interference and object interference conditions, we include different questions regarding the sharing of personal information of the participants (e.g., online social accounts). With these questions, we aim to outline a more realistic scenario and, thus, users' behavior~\citep{distler2021systematic}.

\bparagraph{Questions (object and lighting interference conditions).} We designed the following questions according to the privacy risks that the participants would face in a university environment. We show the participants a website with a leaderboard that includes information about the previous participants, such as their GPA and email. We aim to provide a more realistic environment using these questions and the website. Hence, the participants believe that their results (time) and personal information, such as their GPA and name, will be publicly accessible. The participants can answer yes or no to the following questions:
\label{sec:questions}
\begin{itemize}
    \item Are you willing to share your \textbf{Student ID} with other players at the end of the game?
    \item Are you willing to share your \textbf{GPA} on our web?
    \item Are you willing to share your \textbf{social accounts} on our web?
    \item Would you like to share your \textbf{game ranking} on our web?
    \item Do you agree to allow your \textbf{email} information to start the game?
    \item Are you willing to share your \textbf{phone number} for the researcher to follow up with you?
\end{itemize}

Where the bold keywords are obscured by strong light, all collection processes are fake, but participants are not informed in advance. For all questions, the user only has to select yes or no in the interface.

\bparagraph{Haptic grabbing condition.} The scenario will pop up (at specific locations in the maze) a notification with the following text: \textit{Please press the button below} to confirm the participants have seen the notification, see Figure~\ref{fig:user_study:conditions:haptic}.

% \textcolor{blue}{In haptic grabbing condition, some interfaces will pop up at a specific location in the virtual environment, the text on the interface will ask the participant to press the button, the participant only needs to use the controller to select the "Press" button on the interface.}

\bparagraph{Pilot Study.} We design a pilot study to evaluate the valence and arousal (VA) of the controllers' haptic feedback for VR. The pilot study aims to evaluate the effect on participants' emotions (valence and arousal), driven by the haptic stimuli (i.e., using vibroactuators from the Oculus Quest 2 controller). We design six different haptic feedback following the dark patterns in~\citep{makela2021hidden,yoo2015emotional}. The parameters used to render the vibrotactile feedback are twofold~\citep{rovers2004him}: (I) intensity, three different levels of intensity relative to the default provided by the controller (1) (low (0.5), medium (0.7), high (1)); and (II) frequency, with three different types relative to the default frequency (1) (continuous (1), slow (1/2), and fast (1/4)). We evaluate the responses of nine participants from our university campus (4M/5F, $\overline{age}$ = 21). The participant can experience the same haptic pattern multiple times until they felt that the haptic feedback was completely perceived, at which moment the participant pressed the trigger button on the controller to pop up the Self-Assessment Manikin (SAM) screen~\citep{bradley1994measuring}, which helped the participant determine the emotional feedback at the moment (VA). We select the two most distinctive (according to VA) haptic feedbacks (\textit{happy}, \textit{sad}) for our `haptic grabbing' condition. We aim to study whether an effect on users' behavior exists or not, according to the VA assigned for each of the two selected haptic feedback.



% \subsection{Pilot study - haptic}\label{ssec:pilot}

% We designed a pilot study to evaluate the 

% We designed a pilot study to evaluate the valence and arousal (VA) of the controllers' haptic feedback for VR. The pilot study aims to %With this pilot study we aim to 
% evaluate the effect on participants' emotions (valence and arousal), driven by %according to 
% the haptic stimuli (i.e., using vibroactuators from the Oculus Quest 2 controller). 

% \bparagraph{Design and structure.} We designed six different haptic feedback following the dark patterns in~\citep{makela2021hidden,yoo2015emotional}. The parameters used to render the vibrotactile feedback are twofold: (I) intensity, three different levels of intensity relative to the default provided by the controller (1) (low (0.5), medium (0.7), high (1)); and (II) frequency, with three different types relative to the default frequency (1) (continuous (1), slow (1/2), and fast (1/4)). One of the haptic stimuli is %are 
% inspired by the work~\citep{rovers2004him}, where a gradual increase in the amplitude of the intensity of the vibration is related to %with 
% a positive and pleasant feeling (happy).

% \textbf{Pilot study results.} We recruited 6 participants from our university campus (4M/5F, $\overline{age}$ = 21, high level of education, and average experience with XR applications), where each participant felt in a balanced Latin square order with the six different haptic stimuli as above mentioned. The participant could experience the same haptic pattern multiple times until they %it 
% felt that the haptic feedback was completely perceived, at which moment the participant pressed the trigger button on the controller to pop up the Self-Assessment Manikin (SAM) screen~\citep{bradley1994measuring}, which helped the participant determine the emotional feedback at the %this 
% moment (VA). The results are shown in Figure~\ref{fig:user_study:pilot_study}. From the results of the VA Plot, the haptic feedback can be categorized into B3 that
% %which 
% corresponds to happy and active, and B5 (sad and slow, calm) showed the greatest difference. This is consistent with the prior results in~\citep{yoo2015emotional}. Since the data results did not satisfy the assumptions of ANOVA (not normally distributed), a Friedman test was done on these data, implying that % and the results showed that 
% Valence did not seem to be significantly different, but Arousal has significantly different ($chi-squared = 22.37, df = 5, p <.05$). Additionally, the manual post-hoc pairwise comparisons with paired-samples t-tests found no significance.

% Following the results of the pilot study, we select these two most distinctive (according to VA) haptic feedbacks (B3, B5) for our `haptic grabbing' condition. We aim to study whether %there is an effect on users' behavior 
% an effect on users' behavior exists or not, according to the VA assigned for each of the two selected haptic feedback.




% \textcolor{blue}{6 participants were asked to experience the vibration of the Oculus Quest 2 controllers in a virtual environment, each participant needed to feel 6 haptic patterns (refer to XXX's design), and the order of the participants' experience was disrupted according to the balanced Latin square.}

% \begin{figure}[t]
%   \centering
%     % \begin{subfigure}[b]{0.6\columnwidth}
%     %     \includegraphics[width=\columnwidth]{figures/user_study/Haptic_Pattens.png}
%     %     \caption{.}
%     %     \label{fig:user_study:pilot_study}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.39\columnwidth}
%         \includegraphics[width=0.9\columnwidth]{figures/user_study/VA_Plot.png}
%         \caption{Pilot study results, VA. \textcolor{black}{B3 (happy and active), and B5 (sad and slow, calm) showed the largest differences. These two haptic feedback were chosen as the vibration feedback for the controller in ``haptic garbbing" in the scene \#2 (Sec~\ref{ssec:final-test}).}}
%         \label{fig:user_study:pilot_study}
%     % \end{subfigure}
%     % \caption{.}
%     % \label{fig:user_study:pilot_study}
% \end{figure}

% \textcolor{blue}{}



\subsection{%Formal 
User experiments}

\bparagraph{Task.} Participants were asked %required 
to solve the maze (find the exit) in the shortest time possible. Inside the maze, they had to answer several questions that would appear at particular locations. For the lighting and object interference scenario, the participants responded to 6 questions in Section \ref{sec:questions} in particular locations of the virtual maze. The areas where notifications were triggered are all on the path to the correct maze exit. For the haptic grabbing scenario, participants were requested to press the button in the notification interface they found. The task was accomplished %finish 
when the participants found the exit of the maze or spent more than %2
\textcolor{black}{5} minutes in the maze.



\bparagraph{Procedures.} Participants provided informed consent to participate in this study. Then, we introduced to the participants task and showed them a website that included %includes 
a list of the fastest (fake participants but the participants were not informed.) times to solve the maze. We counterbalanced the order of the three different scenarios. At the end of the experiment, we asked the participants whether they noticed any possible malicious design in the scenarios and asked them to describe them (if any). Finally, the participants responded to demographic-related questions.

The participants took between 16 and 19 minutes to complete the whole experiment. They were rewarded with snacks, sweets, and soft drinks after completion.




% For our study we chose a within-subject design to make participants experience all conditions. 


\subsection{Results}\label{ssec:final-test}

\bparagraph{Lighting and object interference.} We observed that 71.1\% of the responses of the participants were mainly yes when we asked them about sharing any personal information in these virtual scenarios. Only one participant (P12) responded no more times (66.67\%, n=4) than yes (33.33\%, n=2) to the displayed questions. These results show the possible impact of the dark pattern (e.g., lighting interference) on the participants' responses. 

The time participants spend solving the maze and the results of answering the questions in the scene are recorded. Spearman’s rank correlation was computed to assess the relationship between the number of $Yes$ buttons triggered and the time to solve the maze. There was a significant negative correlation between the two variables ($r(13) = -.63, p = .006$). The results are shown in Figure~\ref{fig:user_study:Light_Result}.

\textcolor{black}{12 out of the 15 participants were affected by the bright light on the interactive interface while solving the maze, and 7 of them reported directly to the experimenter that the light made them difficult to read the text. 
%made it difficult for them to read the text. 
Also, the remaining 5 had the behavior of moving around the virtual environment in an attempt to avoid the glare. The dark patterns (object and lighting interference) increase the time that each participant spends answering the questions. When we asked the participants at the end of the experiment whether there was any malicious design in the scenario, 8 participants reported that there was a malicious design. Moreover, 7 of these 8 participants reported the glare/light as the malicious design used in the scenario.
% In the questionnaire responses, 8 people thought there was malicious designs in the scenario, and 7 of them thought the glare/light was malicious design on the immersive interface. 
%the interaction interface. 
Two participants mentioned that the street light in the scene was strange and seemed to have been placed there intentionally, and one of them thought that the street light also obscured the interface.} The participants reported the use of some manipulation techniques when explicitly asked. However, the results show that the participants fell for the malicious design (responding yes to the displayed question).

\begin{figure}[t]
  \centering
    % \begin{subfigure}[b]{0.6\columnwidth}
    %     \includegraphics[width=\columnwidth]{figures/user_study/Haptic_Pattens.png}
    %     \caption{.}
    %     \label{fig:user_study:pilot_study}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.39\columnwidth}
        \includegraphics[width=0.6\columnwidth]{figures/user_study/Light_Result.png}
        \caption{Lighting and object interference results: \textcolor{black}{The time it took participants to find the correct solution to the maze was negatively correlated with the number of times they encountered privacy questions in the maze and triggered the "Yes" button. With
        %, and with 
        glare and objects in the maze, participants who wanted to avoid more privacy risks 
        consuming %wasted 
        their time going through the maze.}}
      
        \label{fig:user_study:Light_Result}
    % \end{subfigure}
    % \caption{.}
    % \label{fig:user_study:Light_Result}
\end{figure}

\bparagraph{Haptic grabbing.} Participants were required to experience two scenes under this condition. 
In each scene, a participant encountered 10 triggered notification (as vibration) with corresponding visual pop-up information (i.e., notification interfaces). %rbtriggered 10 and each scenes participants triggered 10 notification interface. 
Regarding the first scene, % popped up the location of the notification. 
5 out of 10 notification interfaces deliver the vibration on the same side with the visuals being popped up. The remaining half of notification interfaces make opposite direction, i.e., the right-hand-side controller vibrates but notification visuals appear on left-hand side, or vice versa. We note that the participants were informed about the notification interfaces. They had to press the button on the controller to confirm that they spotted the visual notifications. %triggered notification 1/2 is on the same side as the controller (e.g.: the right-hand controller vibration, notification interface from the right side of the participant popped up), 1/2 is on the different side (e.g.: the right-hand controller vibration, notification interface from the left side of the participant popped up). 
Accordingly, the second scene aims to examine the vibration type of positive and negative modes, under the condition of that all ten notification interfaces maintain an opposite direction between the vibration and notification visual. Five of the notification interfaces refer to the positive vibration and the remaining five notification interfaces represent the negative counterpart. Figure~\ref{fig:user_study:Haptic_Exp_Design} shows the details of the scenes setup.  
%was based on our Pilot Study design, where half of the participants triggered the positive mode vibration when they triggered the notification interfaces (see B3 in Section~\ref{ssec:pilot}), and another half of the participants could trigger the negative mode vibration (see B5 in Section 4.2). We note that in this scene, all pop-up notification interfaces and controller vibrations are on different sides. 
In the two above scenes, the number of notification interfaces pressed by the participants was recorded.




\textcolor{black}{%The results of the 
A Shapiro-Wilk test showed that the data satisfied a normal distribution. %,and the results of the 
A one-way ANOVA showed a significant difference in the number of notification interfaces found by participants in the different conditions ($F(3,56) = 5.25, p < .005$). Tukey’s HSD Test revealed that the number of notification interfaces found by participants was significantly higher when the vibration and notification locations were on the same side (SS) than on the different side (DS) condition ($p = 0.005$). In contrast, different vibration haptic patterns did not have a significant effect on the number of notification interfaces that participants were aware of ($p = 0.558$). The results are shown in Figure~\ref{fig:user_study:Haptic_Result}.}

\textcolor{black}{Except for two participants with very serious cybersickness, the remaining 13 participants exhibited the behavior of stopping to look around/seek when the controller vibrated. The results of the questionnaire indicated that 5 participants believed there were malicious designs in the scenario. %, with 4 of them 
Remarkably, 4 of them pointed to vibration as a possible malicious design. One of the participants noted that \textit{"I would unconsciously move in the direction of the controller vibration"}, and another said that \textit{"The controller vibration seemed to manipulate me intentionally"}.}

\begin{figure}[t]
  \centering
    % \begin{subfigure}[b]{0.6\columnwidth}
    %     \includegraphics[width=\columnwidth]{figures/user_study/Haptic_Pattens.png}
    %     \caption{.}
    %     \label{fig:user_study:pilot_study}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.39\columnwidth}
        \includegraphics[width=0.6\columnwidth]{figures/user_study/Haptic_Result.png}
        \caption{Haptic grabbing result, (p $<$ .05 ($\ast$), p $<$ .01 ($\ast\ast$)), where \textit{SS} corresponds to rendering the haptic on the same side as the notification and \textit{DS} to different side. \textit{H1} corresponds to the B3 (happy active), and \textit{H2} to haptic B5 (sad, slow, calm).}

        \label{fig:user_study:Haptic_Result}
    % \end{subfigure}
    % \caption{.}
    % \label{fig:user_study:pilot_study}
\end{figure}

\bparagraph{Post-experiment interview.} We briefly interviewed participants in the questionnaire who believed that light and vibration were malicious designs in the scenario. First, all participants who believed that light was a malicious design agreed that the use of bright light to obscure critical information was an invasion of their privacy, while only one of the participants who believed that vibration was a malicious design considered it to be an invasion of their privacy. In addition, all participants agreed that the vibration design violated their rights. % as users All agreed that the vibration design violated their rights as users. One 
A participant said, \textit{``The vibration design makes me miss information that I am entitled to see''}. All participants agreed that this kind of malicious interaction design is likely to appear in future AR interaction designs. 



%\subsection{Limitations}

%In terms of limitations, using the same physical environment can result in carry-over effects, which can impact the effects of dark patterns. 
%Nevertheless, our study offers a realistic environment to study the effects of dark patterns in AR. One outcome we could not assess with the current study is the long term effect of such dark patterns on users' everyday behavior. Our participants were from our university campus and with relatively experience with XR applications. Therefore, our results should be considered in the context of the participants recruited.


%We use the haptic vibroactuator device embedded in the Oculus controller for our experiment. We agree that further studies in the haptic feedback direction should consider other stimuli areas and different haptic devices. 
%The current user study is a sample of the possibility that dark patterns can have in XR environments. The future version of this work will include more experiments and XR scenarios to provide more in-depth technical details in this direction. 

==> sections/dark_patterns.tex <==
% DArk Patterns
In this section, we describe in more detail the different categories of nudging according to the two taxonomies: the five dark pattern strategies by Gray~\textit{et al.}~\citep{gray2018dark}, and the normative perspectives of dark patterns by Mathur~\textit{et al.}~\citep{mathur2021makes}.


We follow the same taxonomy from Gray\textit{et al.}~\citep{gray2018dark} to categorize the different types of dark patterns (we also include examples of each category):

\begin{itemize}
    \item \textbf{Nagging}, interrupts users' desire for explanation and control. This behavior can be found in applications that interrupt users' flow, including notification messages that pop up while using the application. 
    % In the case of AR scenarios we can think more sophisticated approaches than pop-up notifications (as many AR applications already use). For example, the AR application can request the user to move to a particular spot in the room in order to prompt a specific menu item, which will allow the application to collect more information about the users' environment or diminish the users' motivation to access that menu item due to the movement involved.
    
    \item \textbf{Obstruction},  makes users spend the effort to find and understand an explanation while interacting with explanation or control facilities. We can have examples in the literature of mechanisms such as roach motel (not possible to delete an account), price comparison preview (unable to select the product brand), and intermediate currency (multiple currencies).
    % In the AR environment, the application can request the users to go to a particular physical location in the city to be able to cancel a service or account. 
    
    \item \textbf{Sneaking}, gains from the user's interaction with explanation/control facilities through hidden functions. This technique can force users to agree to accept some data collection practices to unsubscribe from a service. We can enumerate the following examples from literature: sneak into a basket, bait and switch (click a feature that requires a premium account), hidden information, and preselection.  
    % In the case of AR applications, we can see similar approaches forcing users entering a particular retail store in order to unsubscribe a service, increasing the chances of buying something in that retail store. Another example can include the use of augmented objects in the physical world to hide the real cost of items in a store.
    \item \textbf{Interface interferences} encourage explainability or control settings that the system provider prefers. This is one of the most common techniques manifested in interfaces to deceive users when (for example) they agree to the cookie consent notice (with a highlighted accept button). Under this lens, we can observe examples in the real world such as aesthetic manipulation, toying with emotion (countdown offer), false hierarchy, disguised ad (ad appears as normal content in the online newspaper or blog), and trick questions (double negative in the text).
    % In the case of AR scenarios, designers and developers are not limited by interface designs, and can further include physical objects in the surroundings to blend their dark patterns. For example, they can place important (for users) options in a menu (e.g., stop collecting personal information about them) under or behind a physical object so users can not see properly or place these options at the bottom (e.g., on the floor) so they seem less important than the rest. 
    \item \textbf{Forced action} forces users to perform an action before providing them with useful explanations or control options. For example, privacy Zuckering (send usage data preselected) and social pyramid (inviting friends to get access to a special app item).
    % In this strategy we can highlight the use of gamification as it is a common use-case of AR applications, where users are force to do repetitive tasks in order to gain points to pass to the next level of a game. However, in the AR environment, users might require to realize physical movements in order to achieve this points, with the corresponding burden.
\end{itemize}

% The analysis of dark patterns in mobile applications in~\citep{di2020ui} shows that the most common techniques in number of percentage of applications containing each technique are the following: obstruction, sneaking, and interface inferecence.
% Moreover, the nature of AR applications and its usage in the physical world can led users to not only be subjects of undesired data collection practices, but threats about their personal safety (e.g., hide real objects with virtual ones so users will bump into them).

We also follow the taxonomy suggested by Mathur et al.~\citep{mathur2021makes} that the addition of normative perspectives (from other disciplines outside HCI) on dark patterns. The aforementioned taxonomy by~\citep{mathur2021makes} shows guidelines and recommendations to analyze dark patterns outside user interface designs and apply methods grounded in normative perspectives (e.g., psychology, economics, ethics). 
% As we can observe with XR and more particularly AR scenarios such taxonomy will include new aspects that affects individuals' safety under the scope of their individual welfare



\begin{itemize}
    \item \textbf{Individual welfare.} Under this lens, a dark pattern is any interface that modifies the choice architecture to benefit the designer at the expense of the user's welfare.
        \begin{itemize}
            \item \textbf{Financial loss.} Scenarios where dark patterns cause an individual's financial loss, such as in shopping and travel websites. 
            
            % In AR applications designers can use heavy contrast parts of the real world (e.g., highlights or dark spaces) to display the extra charges when purchasing an item or displaying some discounts on physical retails, see example~\ref{}.
            \item \textbf{Invasion of privacy.} Examples of such techniques include difficult to access privacy-respecting choices (e.g., hidden options under cumbersome menus for cookie consent notices). 
            % The continuous sensing of AR applications open new possibilities to collect even more invasive information about users. These applications can force the user to move around their space (e.g., living room) in order to reply to some interface (e.g., signaling them to rotate their phone in order to visualize the notice) while the application is collecting information about the environment (e.g., point cloud, images, objects such as furniture in the room). 
            \item \textbf{Cognitive burden.} We can have examples of such behavior with interfaces that repeatedly prompt the users to accept certain choices or require users to follow cumbersome paths to unsubscribe from a particular service (e.g., via phone). 
            % In the case of AR, applications can include this cognitive burden with difficult to read interfaces (e.g., partially hidden from the users' field of view), therefore users have to move in order to be able to read the whole prompt. 
            % \item safety. This welfare consequence to users is when, in the case of AR scenarios, the dark pattern causes them to harm themselves by hidden real objects (e.g., table) under virtual scenarios, or covering their field of view and forcing them to walk without a fully perspective of the physical world around them.
        \end{itemize}
        
        % In all above scenarios we did not include other techniques that are commonly used in AR applications such as haptics and audio feedbacks. For example, the AR application design can render haptic feedback to users when the interface is prompted, annoying the users and forcing them to accept the default (or predefined) options (cognitive burden). The possibilities with AR applications are broader than other environments such as mobile applications and websites where the 2D interfaces limit the interactions and techniques that dark patterns can use.
        
        
    \item \textbf{Collective welfare.} Normative perspectives such as competition, price transparency, and trust in the market. These dark patterns can tie emotions with products in order to influence users in their purchase decision. 
    % In the case of AR scenarios, designers can display virtual objects such as violent or scary scenes in front of physical retail to influence individuals to not order or buy from that store. As we mentioned above the use of feedback such as audio or haptic when users is nearby a particular place (e.g., retail store) can trigger them emotions (fear) towards it. Therefore, users can have trust issues in similar scenarios that displays virtual objects to attract users' attention honestly. 
    
    % \item Regulatory Objectives
    \item \textbf{Individual autonomy.} Under this lens, a dark pattern is a user interface that undermines individual decision-making. The majority of dark patterns in the literature attempt to undermine individuals' autonomy. 
    % In the case of AR applications, dark patterns can enable even have a broader impact on the autonomy of individuals as such applications are related with real-world behaviours (e.g., freedom of movement). For example, a dark pattern can influence users (`trick') to follow a particular path in the physical world towards a desire destination or virtual object in the augmented space.
\end{itemize}

We omit the normative lens of the regulatory objectives as the regulatory objectives of the AR ecosystem are still under consideration and have limited legal regime scope. For example, the general data protection regulation (GDPR) regulates certain data collection and processing practices. However, despite this regulatory attempt, dark patterns are still a common technique in online services (e.g., websites). This highlights the difficulties regulators have to protect individuals' privacy, whose challenges are even direr in AR scenarios.
